CoHABIT: Complementary Evaluation of Furniture Layouts through Spatial Rules and Household Routines

We introduce CoHABIT, a framework for evaluating furniture layouts through complementary spatial rules and household routines. Static assessment captures geometric validity, ergonomic access, functional organization, and configurable design preferences, including Feng Shui. Dynamic assessment uses learned resident policies to simulate everyday activities, resource sharing, coordination, and individual burdens in multi-agent households. Controlled comparisons show how spatial criteria and household behavior reveal distinct aspects of layout quality, while resident profiles and scheduling influence furnishing rankings. Independent verification of household needs grounds dynamic comparisons in observed outcomes, enabling interpretable assessments of how furnished environments serve different households.

==> figure_tex/pipeline.tex <==

\begin{figure*}[t]\centering
\begin{tikzpicture}[
  font=\small,
  card/.style={draw,rounded corners=2pt,line width=.55pt,
    text width=.29\textwidth,inner xsep=6pt,inner ysep=7pt,align=left},
  flow/.style={-{Stealth[length=4pt,width=3pt]},line width=.5pt,draw=ink!65}]
\node[card,draw=staticblue,fill=staticblue!4] (static) {
  {\color{black}\bfseries Static assessment}\\[4pt]
  $G(L),\ E(L,H)$\\[5pt]
  Geometry and collisions\\
  Use-side access and ergonomics\\
  Functional relationships\\[5pt]
  \emph{Localized criteria}
};
\node[card,draw=preferencepurple,fill=preferencepurple!4,right=8pt of static] (preference) {
  {\color{black}\bfseries Spatial preferences}\\[4pt]
  $F_\rho(L)$\\[5pt]
  Declared spatial principles\\
  Configurable Feng Shui rubric\\
  Rule applicability and context\\[5pt]
  \emph{Criterion-wise ratings}
};
\node[card,draw=dynamicorange,fill=dynamicorange!4,right=8pt of preference] (dynamic) {
  {\color{black}\bfseries Household dynamics}\\[4pt]
  $D_H(L)$\\[5pt]
  Original needs and actions\\
  Costs, waiting and resources\\
  Household interactions\\[5pt]
  \emph{Per-resident outcomes}
};
\node[above=13pt of preference,align=center] (input) {
  Layout $L$, household $H$ and preference rubric $\rho$
};
\draw[draw=ink!65,line width=.5pt] (input.south) -- ($(preference.north)+(0,6pt)$);
\draw[draw=ink!65,line width=.5pt] ($(static.north)+(0,6pt)$) -- ($(dynamic.north)+(0,6pt)$);
\draw[flow] ($(static.north)+(0,6pt)$) -- (static.north);
\draw[flow] ($(preference.north)+(0,6pt)$) -- (preference.north);
\draw[flow] ($(dynamic.north)+(0,6pt)$) -- (dynamic.north);
\node[draw=rulegray,rounded corners=2pt,fill=ink!3,text width=.94\textwidth,
  inner xsep=6pt,inner ysep=7pt,align=center,below=14pt of preference] (quality) {
  \mbox{$\mathcal Q(L,H,\rho)=\bigl(G(L),E(L,H),F_\rho(L),D_H(L)\bigr)$}\\[3pt]
  Distinct criteria, need outcomes and costs remain inspectable.
};
\draw[flow] (static.south) -- (static.south |- quality.north);
\draw[flow] (preference.south) -- (quality.north);
\draw[flow] (dynamic.south) -- (dynamic.south |- quality.north);
\node[below=7pt of quality,align=center,text width=.96\textwidth,font=\footnotesize] {
  \textbf{Optional feasibility verdict:} required geometry AND verified dynamic contract.\\
  This scoped positive/negative/unknown readout is separate from the assessment vector.
};
\end{tikzpicture}
\caption{\textbf{Complementary assessment of one layout.} Geometry, declared preferences and household execution retain separate criteria, coverage and uncertainty. Certification checks required constraints and needs.}
\label{fig:pipeline}
\end{figure*}


==> figure_tex/vlm_examples_3d.tex <==

\begin{figure*}[!tp]\centering
\begin{minipage}[c][\textheight][c]{\textwidth}\centering
\includegraphics[width=.99\textwidth]{figures/vlm_access_examples_3d.pdf}
\caption{\textbf{Orientation and doorway access explain individual judge disagreements.} (a) Rotating the sink preserves its footprint but turns its working side toward the wall. (b) Moving the sofa obstructs two door-clearance zones. Blue arrows show facing; dashed rectangles mark clearance zones whose depth equals the door width. Red marks footprint intersections. Each pair shares camera, scale, materials and lighting. Footprints, orientations and openings come from the original JSON; heights and materials provide illustrative 3D context. Rule penalties aggregate the whole apartment; lower is preferred. The VLM judge is the argon endpoint in Table~\ref{tab:static-by-kind}. Displayed judge decisions use the original 2D plans; the 3D views reconstruct their geometric context.}
\label{fig:vlm-access-3d}
\end{minipage}
\end{figure*}

\begin{figure*}[!tp]\centering
\begin{minipage}[c][\textheight][c]{\textwidth}\centering
\includegraphics[width=.99\textwidth]{figures/vlm_overlap_examples_3d.pdf}
\caption{\textbf{Local geometric evidence and aggregate ordering provide different information.} (a) A 45\,cm table shift creates a small footprint intersection with a chair, detected by the rules while the VLM judge prefers the edit. (b) The critic detects both new sofa/table overlaps, yet its aggregate penalty falls from 38 to 37; the visual judge prefers the control. The plan insets expose intersections that are partly occluded in 3D. Areas measure intersections of projected object footprints. Rendering and decision provenance follow Figure~\ref{fig:vlm-access-3d}. These selected cases illustrate mechanisms; aggregate performance is reported in Table~\ref{tab:static-by-kind}.}
\label{fig:vlm-overlap-3d}
\end{minipage}
\end{figure*}


==> supplement_sections/a_setup.tex <==
\section{Assessment Inputs and Interpretation}
\label{app:evidence_boundaries}\label{app:reporting_model}\label{app:framework}
A layout $\mathcal{L}=(\Omega,\{B_j,\alpha_j,z_j,\mathcal A_j\}_j,\mathcal D)$ contains metric rooms, furniture footprints, facing, height, affordances and openings. Household $H$ declares movement, reach and carrying capabilities; a scenario fixes original semantic needs, dependencies, releases, deadlines and shared resources. Each matched furnishing comparison preserves envelope, inventory, household, physical starts, original needs, thresholds and exogenous random draws. A profile intervention changes the declared profile while holding the furnishings fixed.
\input{figure_tex/pipeline}

\subsection{Profiles and population}
\label{app:resident-profiles}
The rich furnishing corpus uses standard+fast and standard+wide-clearance households. Daily kitchen comparisons use standard+standard and standard+slow. The reference gallery uses the rich-corpus profiles. Each furnishing pair retains its original ordered household. The static perturbation study instead uses a fixed 0.25\,m navigation radius and 0.10\,m grid.
\begin{table}[t]\centering\small
\caption{Profiles used in the reported cohorts. Lengths are metres; speed is m/s. Each resident carries one portable object. Int. denotes interaction reach.}
\label{tab:resident-profiles}
\begin{tabular}{@{}lrrrrr@{}}\toprule
Profile & Radius & Speed & Reach & Int. & Height\\\midrule
Standard & .25 & 1.20 & 1.50 & .85 & 1.72\\
Fast & .25 & 1.55 & 1.50 & .85 & 1.72\\
Wide-clearance & .40 & .90 & 1.40 & .85 & 1.65\\
Slow & .28 & .65 & 1.40 & .80 & 1.70\\\bottomrule
\end{tabular}\end{table}
Fast changes speed only. Wide-clearance changes radius, speed, reach and stored height together; its contrast is a compound capability intervention. NAV radius determines graph clearance, speed determines traversal duration and reach determines height eligibility. These quantities parameterize the logical simulation. Daily kitchen comparisons replace B's standard profile with the slow capability bundle while holding resident A standard. This intervention jointly changes radius, speed, reach, interaction reach and stored height.

\begin{figure*}[t]\centering
\includegraphics[width=\textwidth]{figures/cohabit_household_compositions.pdf}
\caption{\textbf{Declared household compositions and comparison inputs.} Solo and two-resident furnishing contexts are separate from the two-adult-plus-child family series. Each comparison fixes original needs, numerical profiles, calendars and starts, and preserves individual outcomes and costs. Characters and calendar bars schematically identify resident roles and request timing; numerical parameters define the simulated capabilities.}
\label{fig:household-compositions}
\end{figure*}

\subsection{Criteria, needs and verdicts}
Static findings retain criterion identity, applicability, value and affected objects. Dynamic findings retain each resident's original required, met, independently verified-unmet and unresolved needs, together with distance, instrumental time, waiting, deadlines and conflicts. A semantic need is an AND of its required predicates; actions and needs have distinct denominators.

An applicable unavailable criterion is $\bot$; an inapplicable criterion is NA. Coverage is the measured applicable fraction and is undefined for an empty denominator. Each missing value retains its explicit availability state. A positive feasibility verdict requires every original required need and fixed cost limit to be verified. A supported adverse verdict requires a necessity certificate or justified cost attribution under competent execution. Policy loops and unsupported bindings remain unresolved unless independent adverse evidence applies.

The optional certification gate conjoins required geometry with verified dynamic conditions: supported failure prevails, positive requires both branches positive, otherwise the verdict is unknown. G, E, F and D remain separate reports; required failures determine the feasibility gate independently of preferences.


==> supplement_sections/b_static.tex <==
\section{Static Criteria and Perturbation Evidence}
\label{app:static_track}
\label{app:hanfu}

\begin{figure*}[tp]\centering
\includegraphics[width=\textwidth]{figures/cohabit_static_algorithm_v2.pdf}
\caption{\textbf{Static assessment preserves the source and meaning of every criterion.} The source-derived bedroom view shows the tested rotation/translation case. The evaluator retains coordinates and facing, measures geometric and use-side relations, and reports availability and localized witnesses. Required predicates, recommendations and optional spatial preferences remain distinct. The depicted physical preference checks refer to the five-criterion geometric implementation used in our experiments; the complete ten-criterion HANFU rubric is defined below.}
\label{fig:static-algorithm}
\end{figure*}

\subsection{Geometry, ergonomic rules and missing criteria}
For observed metric geometry, example hard predicates are
\begin{align}
h^{\rm inside}_j&=\ind[B_j\subseteq\Omega_{\rm room(j)}],\nonumber\\
h^{\rm overlap}_{jk}&=\ind[\operatorname{area}(B_j\cap B_k)\leq\epsilon_{jk}],
\label{eq:geometric-predicates}
\end{align}
where the overlap test excludes permitted support and containment contacts. Tolerances and contact semantics are declared. Facing-dependent access envelopes use $\alpha_j$ to distinguish orientations with identical footprints. An operational-clearance criterion needs a declared use direction and body profile, together with a sourced threshold. Numerical ergonomic criteria require explicit thresholds, applicability and source references; illustrative drawings supply geometric context.

For measurement $c_j(\mathcal{L},p)$, a declared map gives $s_j=\psi_j(c_j;p)$. A possible clearance map is $\psi_j(d;p)=\operatorname{clip}(d/\eta_j(p), 0, 1)$, but $\eta_j(p)$ still requires grounding. An ordinal $K_j$-level preference can use $(c_j-1)/(K_j-1)$. Each normalized score retains its criterion-specific meaning.

Record applicability $a_j$ and availability $m_j$ using the missingness conventions in Appendix~A. For a nonempty set $\mathcal H_p$ of applicable required hard checks,
\begin{equation}
G_{\rm req}=\begin{cases}
\mathrm{FAIL},&\exists j\in\mathcal H_p:m_j=1,\ h_j=0,\\
\mathrm{PASS},&\forall j\in\mathcal H_p:m_j=1,\ h_j=1,\\
\mathrm{UNKNOWN},&\text{otherwise}.
\end{cases}
\label{eq:hard-status}
\end{equation}
An unspecified check set is UNKNOWN. Criterion coverage is $\sum_ja_jm_j/\sum_ja_j$, unavailable when the denominator is empty. Unknown values retain a distinct status. Hard failures receive localized diagnoses; soft ergonomic deficits and preferences remain inspectable. Comparisons among passing layouts use the same criterion and household contract and retain tradeoffs.

\input{supplement_sections/b_static_methods}

\subsection{Static controls and edits}
The static set contains 50 furnished controls with six edits each: shift, $180^\circ$ orientation change, door blocking, overlap, wall crossing and combined edits. Thus it contains 350 scenes and 300 control--edit pairs. Apartments have 4--8 rooms, 17--35 objects and 44.01--100\,m$^2$ area. They derive from 19 source layouts in 11 outer-contour families. The supplied split has 37/5/8 controls across 8/1/2 train/validation/test families.

These data were collected for static assessment. Their furnishing briefs specify static design conditions; dynamic residents use separately declared simulator profiles. Edit labels specify intended local degradation relative to the selected controls. Some edits introduce several defects. An evaluator should therefore report pair preference, ties and object-level diagnosis separately. Local finding detection and aggregate pair ordering are evaluated separately.

\begin{table}[t]\centering\small
\caption{Audit of supplied static annotations; each row has 50 scenes. Counts report scenes with at least one stored violation.}
\label{tab:static}
\begin{tabular}{@{}lrrr@{}}\toprule
Edit & Overlap & Opening & Outside\\\midrule
Control &0&0&0\\
Shift &50&2&0\\
Orientation $180^\circ$ &0&0&0\\
Door block &0&50&0\\
Overlap &50&10&0\\
Wall crossing &9&4&50\\
Combined &50&39&0\\\bottomrule
\end{tabular}\end{table}
All 50 orientation edits preserve the three geometry checks in Table~\ref{tab:static}. Their stored front-blocking diagnostic increases from .3170 to .3700 on average (paired difference +.0530). This quantifies orientation-sensitive use-side access at unchanged footprints.

\input{supplement_sections/b_static_results}

\subsection{Optional preference criteria}
HANFU is the spatial-preference rubric of CoHABIT, complementing its physical-feasibility assessment. Combining scores requires compatible context and criterion meanings.
\begin{table}[t]\centering\small
\caption{CoHABIT's ten-criterion HANFU rubric. Each rating uses explicitly supplied contextual attributes.}
\begin{tabularx}{\linewidth}{@{}lYl@{}}\toprule
ID & Criterion & Scale\\\midrule
F1 & Bed commanding position & 1--4\\
F2 & Desk commanding position & 1--4\\
F3 & Sofa commanding position & 1--3\\
F4 & Bagua alignment & 1--4\\
F5 & Kitchen positioning & 1--4\\
F6 & Directed-corner/alignment avoidance & 1--3\\
F7 & Door--bed alignment & 1--2\\
F8 & Mirror placement & 1--2\\
F9 & Elemental balance & 1--3\\
F10 & Yin--yang zoning & 1--3\\\bottomrule
\end{tabularx}\end{table}
Commanding-position criteria require orientation, entrance and backing geometry; directional criteria need compass bearing and declared sectors; mirror and material criteria need corresponding attributes. Incompatible legacy meanings, especially F5, prevent criterion-level comparison across implementations.

For fixed active, applicable criteria $\mathcal A_p$ and declared nonnegative weights, an optional summary requires every active rating:
\begin{equation}
F_p(\mathcal{L})=\frac{\sum_{c\in\mathcal A_p}w_c(s_c-1)}{\sum_{c\in\mathcal A_p}w_c(K_c-1)}.
\end{equation}
A missing active rating or zero denominator yields an unavailable scalar while preserving the fixed active set. Reports retain the vector, active set, missingness and coverage. Changing that set changes the interpretation. The five-criterion results above measure agreement with that rubric and its synthetic targets; HANFU retains its own criterion definitions.

\begin{center}
\includegraphics[width=\linewidth]{figures/panelF.pdf}
\captionof{figure}{\textbf{The source geometry behind the main-paper headboard example.} A $180^\circ$ bed rotation preserves every furniture footprint, room and opening of the eight-room control. The explicit F1 headboard-support subrule changes: oriented rear-edge contact with the solid room boundary falls from 1.68\,m to zero (openings excluded; $10^{-6}$\,m tolerance). This local geometric witness is separate from ordinal five-criterion ratings and the 48-pair comparison.}
\label{fig:headboard-source}
\end{center}

\paragraph{Motivating example: clearance and routine completion.}
Figure~\ref{fig:chair-clearance-3d} shows the same apartment before and after a furnishing intervention: the critic's dining-chair clearance decreases from 0.64 to 0.44\,m. The implemented 0.60-m chair-use threshold is satisfied only in A; neither meets its 0.80-m recommendation for passage behind a seated person. Both layouts complete the declared routines (Appendix~H), while the reduced clearance changes the space available for using the chair. This motivates complementary spatial and temporal assessment on the same furnishings. Figure~\ref{fig:vlm-access-3d} provides complementary sink-facing and door-zone examples.
\begin{figure*}[tp]\centering
\begin{minipage}{.48\textwidth}\centering
\textbf{A: wider chair-use clearance}\\
\includegraphics[width=\linewidth]{figures/clearance_room_A_annotated.pdf}\\
Measured clearance: 0.64\,m
\end{minipage}\hfill
\begin{minipage}{.48\textwidth}\centering
\textbf{B: narrower chair-use clearance}\\
\includegraphics[width=\linewidth]{figures/clearance_room_B_annotated.pdf}\\
Measured clearance: 0.44\,m
\end{minipage}
\caption{\textbf{Geometric clearance adds information beyond completed routines.} Source-bound 3D views of apartment 026 under the living-room intervention in Appendix~H. Dimension arrows mark the table-edge-to-sofa clearance across the chair-use zone; 0.64\,m in A meets the implemented 0.60-m chair-use threshold, whereas 0.44\,m in B does not. The 0.80-m recommendation for passage behind a seated person is unmet in both. The camera, scale and lighting are shared; footprints and orientations follow the evaluated JSON, while materials and heights are illustrative. Both variants complete the household routine; the narrower chair-use space illustrates the additional information supplied by ergonomic checks.}
\label{fig:chair-clearance-3d}
\end{figure*}


==> supplement_sections/b_static_methods.tex <==
\subsection{From geometric measurements to criterion reports}
Figure~\ref{fig:static-algorithm} traces the implemented measurements from furnished geometry to separate G, E and preference records. Algorithm~1 makes applicability, availability and the original rubric explicit. $G$ is computed from the required checks only, whereas $E$ aggregates all findings of the geometry/ergonomics critic, including recommendations. Proposed repairs are evaluated as new layouts, checking both resolved and newly introduced findings.



\begin{table*}[t]\centering\small
\begin{tabularx}{\textwidth}{@{}rY@{}}\toprule
\multicolumn{2}{@{}l}{\textbf{Algorithm 1. Static criteria with explicit availability}}\\\midrule
\textbf{Input}&Furnished geometry $\mathcal{L}$, household $H$, preference rubric $\rho$, criterion registry $\mathcal R$.\\
\textbf{Output}&Separate reports $G,E,F_\rho$ and localized evidence records $\mathcal Z$.\\\midrule
1&$\widehat{\mathcal{L}}\gets\operatorname{Normalize}(\mathcal{L})$; retain coordinates, facing, supports and source-opening correspondence.\\
2&$\mathcal Z\gets\varnothing$.\\
3&\textbf{for each} criterion $r\in\mathcal R$ \textbf{do}\\
4&\quad Determine applicability from $(\widehat{\mathcal{L}},H,\rho)$; record inactive criteria without scoring them.\\
5&\quad \textbf{if} required attributes are unavailable, append an unavailable record and \textbf{continue}.\\
6&\quad $m_r\gets\operatorname{Measure}_r(\widehat{\mathcal{L}},H)$ with declared units and geometry tolerances.\\
7&\quad $v_r\gets\operatorname{Evaluate}_r(m_r;\rho)$; retain the measured fact, rule source and affected objects.\\
8&\quad Append $(r,m_r,v_r,\mathrm{source},\mathrm{availability},\mathrm{witness})$ to $\mathcal Z$.\\
9&$G\gets\operatorname{RequiredVerdict}(\mathcal Z)$ using only records of required checks: verified failure dominates; otherwise missing required evidence yields UNKNOWN.\\
10&$E\gets3n_{\mathrm{critical}}+n_{\mathrm{advisory}}$ over geometry/ergonomics findings in $\mathcal Z$, including hard checks and recommendations; retain the full finding list.\\
11&$F_\rho\gets\operatorname{PreferenceReadout}(\mathcal Z;\rho)$ with fixed active criteria and versioned aggregation.\\
12&\textbf{return} $(G,E,F_\rho,\mathcal Z)$; a proposed repair must be evaluated as a new layout.\\\bottomrule
\end{tabularx}
\end{table*}


==> supplement_sections/b_static_results.tex <==
\subsection{Static comparison protocol}
\label{app:static_archive_evidence}
\textbf{Reported} values are archive summaries; \textbf{rechecked} values are recomputed from individual records; \textbf{post-hoc} comparisons reuse the inspected pairs. Pair accuracy awards one for preferring the control, one half for a tie and zero otherwise. Strict correctness excludes ties. Detection counts new critical findings; localization checks the changed object; repair counts removed findings. These are distinct targets.

The selected corpus contains 50 furnished controls from 19 source layouts and 11 contour families, with six edits per control. The training/validation/test splits contain 222/30/48 pairs, 37/5/8 controls and 8/1/2 contour families. The test controls come from three source layouts; six controls share one contour family and two share the other. Counts refer to the selected controls.

The geometry/ergonomics critic ranks by $3n_{\rm critical}+n_{\rm advisory}$, lower being better. SceneEval~\cite{tam2026sceneeval} and SceneSmith~\cite{pfaff2026scenesmith} supply the archived baseline comparisons. The VLM judge uses the recorded gemini-4-argon endpoint (alias argon) to view plans with icons and randomized A/B order. The static--VLM cascade queries its judge when the rule-score gap is below three, approximately 20\% of pairs. It combines two static instruments.

\subsection{Reported ranking, localization and repair}
Tables~\ref{tab:static-full-ranking} and~\ref{tab:static-by-kind} give the full comparison and edit-specific values.
\begin{table}[t]\centering\small
\setlength{\tabcolsep}{3pt}
\caption{\textbf{Reported} pair accuracy (half-credit ties) and strict correctness. All: 300 pairs; Test: 48 pairs. Unreported strict values use --.}
\label{tab:static-full-ranking}
\begin{tabular}{@{}lrrr@{}}\toprule
Method & All & Test & Strict (all)\\\midrule
Geometry/ergonomics & .917 & .958 & .883\\
SceneEval COL & .770 & .771 & .543\\
SceneEval OOB & .555 & .542 & .110\\
NAV 0.2\,m & .408 & .312 & .287\\
NAV 0.6\,m & .478 & .583 & .373\\
ACC side table & .667 & .625 & .573\\
ACC VLM sides & .627 & .521 & .563\\
Door zones & .663 & .698 & .337\\
Window zones & .500 & .500 & .000\\
SceneSmith reach 0.3\,m & .547 & .479 & .307\\
SceneSmith reach 0.6\,m & .572 & .635 & .350\\\midrule
Reimpl. collision fraction & .778 & .771 & .557\\
Reimpl. out-of-bounds & .555 & .542 & .110\\
Reimpl. overlap rate & .778 & .771 & .560\\
Reimpl. orientation & .605 & .667 & .220\\
Reimpl. reachable rate & .637 & .604 & .347\\\midrule
VLM judge & .948 & .948 & \NM\\
Static--VLM cascade & .983 & .990 & \NM\\\bottomrule
\end{tabular}\end{table}

Table~\ref{tab:static-full-ranking} evaluates all instruments on the six local-edit types; the baseline methods originate in generator-comparison settings. A finding can be detected while other penalties reverse the aggregate ranking. The critic reports .98 finding detection, .917 half-credit pair accuracy and .883 strict pair accuracy, each with its stated target. Table~\ref{tab:static-by-kind} uses the same half-credit metric in every cell. The window-zone baseline ties every pair: half-credit accuracy .500 with strict correctness .000.

\begin{table}[t]\centering\small
\setlength{\tabcolsep}{3pt}
\caption{\textbf{Reported} half-credit accuracy by edit, 50 pairs per row. Cascade combines the rule critic with the same VLM judge.}
\label{tab:static-by-kind}
\begin{tabular}{@{}lrrr@{}}\toprule
Edit & Rules & VLM & Cascade\\\midrule
Shift & .88 & .96 & \textbf{.98}\\
Rotation & .95 & .78 & \textbf{.96}\\
Door block & .95 & .98 & \textbf{1.00}\\
Overlap & .85 & \textbf{1.00} & \textbf{1.00}\\
Wall crossing & .87 & \textbf{.99} & .96\\
Combined & \textbf{1.00} & .98 & \textbf{1.00}\\\bottomrule
\end{tabular}\end{table}

\paragraph{Error mechanisms in preserved examples.}
On rotations, rules improve on the VLM judge from .78 to .95 and the cascade reaches .96. Figures~\ref{fig:vlm-access-3d}--\ref{fig:vlm-overlap-3d} reconstruct four preserved comparisons: working-side orientation, door-zone obstruction, a table/chair intersection, and sofa/table overlaps. The first three show how local geometric measurements explain individual disagreements between rules and the visual judge. The fourth separates diagnosis from ranking: the critic detects overlaps but its aggregate penalty prefers the edit. These selected examples explain mechanisms; category frequencies are reported in Table~\ref{tab:static-by-kind}. Use-side clearance has no separately scored category beyond these rotation examples. The displacement-dose test below evaluates the rule critic only.

\input{figure_tex/vlm_examples_3d}

\paragraph{External-query cost.}
The local rule critic makes no external API requests. At the recorded approximately 20\% judge-call rate, the cascade uses about 80\% fewer requests than judging every pair. Historical archive estimates are approximately \$0.008 per pair for the VLM judge and \$0.0015 for its cascade. Five saved examples retain per-response charges of \$0.00638--0.00792. These recorded estimates and response charges characterize historical API expense; matched local CPU cost is outside this comparison.

\paragraph{Reported uncertainty.}
The archived bootstrap uses 4,000 resamples of the 50 generated controls, carrying all six edits with each selected control (random seed 0). Its reported 95\% intervals are critic .917 [.888,.945], VLM judge .948 [.927,.967] and cascade .983 [.970,.993]. These intervals, reproduced in the main table where available, describe variation over generated controls, conditional on the selected source geometry; they include training and validation controls. Controls are resampled with their six edits; source layouts and contour families are not resampling units. Table~\ref{tab:static-paired-ci} preserves the archived paired differences. The 48-pair test gives a descriptive comparison of observed scores on two held-out contour families.

\begin{table}[t]\centering\small
\caption{\textbf{Reported} paired differences on 300 pairs, with 95\% intervals resampling the 50 generated controls. See the stated conditional uncertainty scope.}
\label{tab:static-paired-ci}
\begin{tabular}{@{}lrr@{}}\toprule
Comparison & Difference & 95\% interval\\\midrule
Critic minus VLM & $-.032$ & [$-.065,.002$]\\
Cascade minus VLM & $+.035$ & [.017,.055]\\\bottomrule
\end{tabular}\end{table}

The critic--VLM difference interval spans zero. The cascade--VLM interval is positive under the stated control-level resampling. The recorded strict-correctness McNemar tests operate at pair level. Probabilities displayed as zero are rounded values. These pair-level summaries leave geometry-clustered significance unevaluated.

\paragraph{Reported object-level diagnosis and repair.}
New findings name the changed item in 243/250 single-defect pairs. A new critical finding appears in 294/300 pairs; these pairs yield 560 new findings, of which 64\% reportedly have an automatic fix. Three rounds remove 422/560 findings (75.36\%; Table~\ref{tab:static-repair}). The reported 16\% repair-regression figure is retained as a summary statistic with an unspecified event denominator. Each repaired layout requires a full reassessment of resolved and newly introduced findings. The 141/273 slide-summary count and 422/560 finding count describe separate runs and are reported separately.

\begin{table}[t]\centering\small
\caption{\textbf{Reported} new findings and removals after three rounds. The counting unit is an individual finding.}
\label{tab:static-repair}
\begin{tabular}{@{}lrr@{}}\toprule
Edit & New findings & Removed\\\midrule
Shift & 93 & 82\\
Rotation & 47 & 47\\
Door block & 82 & 77\\
Overlap & 85 & 41\\
Wall crossing & 71 & 42\\
Combined & 182 & 133\\\midrule
\textbf{Total} & 560 & \textbf{422}\\\bottomrule
\end{tabular}\end{table}

\subsection{Post-hoc check selection and score diagnostics}
\label{app:static_posthoc}
The ablation tables separate check selection, individual contributions and scalar weighting; their common limitation is reuse of the inspected pairs.
\textbf{Exploratory analysis on the inspected pairs.} The hard-plus-orientation subset in Table~\ref{tab:static-posthoc} was selected on these pairs. Its .983 overall and .990 test-subset scores therefore describe post-hoc performance on reused data. Here ``hard'' denotes implemented collision, out-of-bounds and door/window checks; required resident conditions have a separate definition. The scalar assigns critical severity to some recommendations, including gaps; household applicability is specified separately. The archive retained the gap check despite its adverse ranking delta. Recommendation checks require further grounding even when they improve synthetic edit ranking.

\begin{table}[t]\centering\small
\caption{\textbf{Post-hoc reported diagnostics} on the same 300 pairs; half-credit ties. The selected subset also reports .990 on the reused 48-pair test subset, without independent selection.}
\label{tab:static-posthoc}
\begin{tabular}{@{}lrr@{}}\toprule
Findings scored & All & Rotation (50)\\\midrule
Hard checks only & .912 & .50\\
Recommendations only & .618 & .95\\
Orientation only & .662 & .95\\
Hard plus orientation (selected) & \textbf{.983} & .95\\
All checks (main comparison) & .917 & .95\\\bottomrule
\end{tabular}\end{table}

Reported leave-one-check-out changes in pair accuracy are collision $-.108$, opening clearance $-.092$, orientation $-.075$, out-of-bounds $-.062$, bed access $-.003$, door reachability $-.002$, dining-chair space $+.005$, navigability $+.007$ and gap violations $+.062$; the other nine checks change the rounded score by zero. A zero delta records unchanged aggregate accuracy on these interventions. Critical:advisory weights 1: 1, 2: 1, 3: 1, 5: 1 and 10: 1 give .862, .905, .917, .917 and .917; critical-only scoring gives .930. These same-data diagnostics measure sensitivity to aggregation and preexisting control penalties; validation of alternative weights requires a separate selection-and-test protocol.

\subsection{Reported judge stability and findings assistance}
Repeated-judge results cover a 90-pair subset (Table~\ref{tab:static-repeats}). Similar aggregate accuracy can coexist with changes in individual verdicts.

\begin{table}[t]\centering\small
\caption{\textbf{Reported} repeat stability. Agreement is the fraction retaining the same verdict across the listed repeats.}
\label{tab:static-repeats}
\begin{tabular}{@{}lrrl@{}}\toprule
Judge & Pairs & Repeats & Accuracy; agreement\\\midrule
VLM judge & 90 & 2 & .944, .933; .978\\\bottomrule
\end{tabular}\end{table}

Providing critical findings defines an additional prompt condition under the same evaluation labels. The reported matched-subset results are in Table~\ref{tab:static-findings}. The all-pair subsets differ from 300 and their test slices differ from 48. Orientation accuracy changes from .793 to .939 (41 pairs). On the 42-pair test slice, the aggregate score remains unchanged. On the all-pair matched subset, cascade accuracy decreases from .9826 to .9807 with findings assistance. Repeat and assisted-prompt results use the saved summary statistics.

\begin{table}[t]\centering\small
\caption{\textbf{Reported} findings-assisted judge accuracy and ties on matched subsets. Test rows are nested subsets of the corresponding all rows.}
\label{tab:static-findings}
\begin{tabular}{@{}llrrr@{}}\toprule
Judge & Subset ($n$) & Base & Findings & Ties, base$\to$new\\\midrule
VLM & All (259) & .9498 & .9826 & 18$\to$5\\
VLM & Test (42) & \textbf{.9524} & \textbf{.9524} & 4$\to$2\\\bottomrule
\end{tabular}\end{table}

\subsection{Arithmetic recheck: shift-dose records}
We independently recomputed Table~\ref{tab:static-dose} from 200 supplied individual records: the same 50 controls at each of four displacement magnitudes. This recheck verifies arithmetic and denominators of the saved checker outputs. Pair ordering reflects displacement alongside all other scored penalties. Target objects and directions are selected using overlap at the largest tested displacement. The displacement-dose evaluation covers the rule critic.

\begin{table}[t]\centering\small
\caption{\textbf{Arithmetic rechecked from saved checker outputs}. Each magnitude has 50 pairs; accuracy credits ties by one half, detection counts a new critical finding.}
\label{tab:static-dose}
\begin{tabular}{@{}lrr@{}}\toprule
Displacement & Pair accuracy & Detection\\\midrule
0.05\,m & .77 & .56\\
0.10\,m & .86 & .82\\
0.20\,m & \textbf{.93} & \textbf{.98}\\
0.40\,m & .92 & \textbf{.98}\\\bottomrule
\end{tabular}\end{table}

\subsection{Preference experiments and criterion definitions}
\label{app:five_criterion_preferences}
The five-criterion spatial-preference rubric defines F1 backing support, F3 entrance view, F5 circulation, F7 angle exposure and F10 density. These criterion definitions and results are reported separately from the complete HANFU rubric below. Its results measure agreement with synthetic interventions under those definitions.

From the supplied 48 test-pair records and 98 scene-status records, we recomputed image-based argon preference accuracy .7292, geometry-based preference accuracy .5833 and ergonomics accuracy .9583. The ergonomics-first, image-preference-on-ties tandem scores .979, resolving two critic ties; it is comparable to the .958 critic on this small subset. Image preference scores .375 on the eight shift pairs. This task scores scenes under the preference rubric, whereas the main table's judge compares ergonomic edits directly.

Rechecking the archived results gives geometry-preference/ergonomics/tandem accuracies of .560/.917/.918 on 300 ergonomic pairs and .704/.621/.723 on 157 preference-targeted pairs. The records are available from the authors. These saved evaluations use an earlier ergonomics-critic version and reveal sensitivity to criterion choice. The image comparison uses one VLM on eight test controls, with 48 paired interventions. The reported scene-score correlation $r=.33$, approximately 3.5 attempts per valid image response and 44\% unrated criteria likewise lack complete independent regeneration. Output validity, scene judgment and criterion coverage are recorded as distinct quantities.

\begin{table}[t]\centering\small
\caption{\textbf{Reported room-level exact agreement} between geometry and image modes of the experimental preference implementation. Counts are transcribed from the reported room-rating summaries.}
\label{tab:static-preference-agreement}
\begin{tabular}{@{}llrr@{}}\toprule
ID & Preference criterion & Agree / total & \%\\\midrule
F1 & Backing support & 60/106 & 56.6\\
F3 & Entrance view & 56/98 & 57.1\\
F5 & Circulation & 197/401 & 49.1\\
F7 & Angle exposure & 61/106 & 57.5\\
F10 & Density & 275/401 & \textbf{68.6}\\\bottomrule
\end{tabular}\end{table}



\subsection{Record provenance}
Reported rankings, detection, localization, repair and judge statistics are transcribed from their respective archive summaries. Arithmetic checks cover the 200 displacement comparisons, the 48-pair preference test, and the 300- and 157-pair preference/ergonomics comparisons. These evidence types retain separate labels throughout the section. The measured figures use the corresponding static records; dynamic rollout figures use recorded apartment executions.


==> supplement_sections/c_architecture_learning.tex <==
The resident computation in Figure~\ref{fig:architecture-detailed} is bound to the pinned daily implementation. Schematic residents denote separately acting decision makers with shared weights. Their actions change one persistent apartment state; original-need assessment is independent of the training objective. The 3D thumbnail reuses exact source furnishing geometry with illustrative materials and heights.

\begin{figure*}[tp]\centering
\includegraphics[width=\textwidth]{figures/cohabit_architecture_v2_detail.pdf}
\caption{\textbf{Learned resident computation and shared-world semantics.} The two-resident daily architecture is shown from its pinned implementation. Request selection uses embedded released needs, prerequisite-neighbor aggregation and current context; the selected request conditions the shared pre-norm Transformer. Object-wise action logits are masked before fixed decoding. The three-resident model has a separate smaller backbone and extends the interface with recipient-specific transfer choices. The lower panels distinguish the BC actors used in the daily/family studies from the separately recorded MAPPO training protocol. Independent household readout uses executed events and the declared assessment functional.}
\label{fig:architecture-detailed}
\end{figure*}

\subsection{Learning objectives and implemented architecture}
\label{app:architecture-learning}
For recorded MAPPO studies, residents share an actor while a separate centralized value critic conditions on the joint state. With importance ratio $r_{n,i}(\theta)$ and a critic-derived advantage $\widehat A_{n,i}$, the actor uses the clipped PPO objective
\begin{equation}
\begin{aligned}
\mathcal L_{\rm clip}(\theta)=\mathbb E_{n,i}\big[\min\big(&r_{n,i}(\theta)\widehat A_{n,i},\\
&\operatorname{clip}(r_{n,i}(\theta),1-\epsilon,1+\epsilon)\widehat A_{n,i}\big)\big].
\end{aligned}
\end{equation}
The implementation's time-aware discounts and current-state value estimates account for variable-duration events. The actor and critic learn during training; fixed resident policies generate evaluation trajectories. Centralized value information supports learning from interacting decisions in a common state~\cite{yu2022mappo,ppo2017}.

The successful daily and family comparison actors instead optimize masked request/action cross-entropy on constructive demonstrations:
\begin{equation}
\begin{aligned}
\mathcal L_{\rm BC}= -\mathbb E_{(o,q^*,a^*)}\!\big[&w_q\log\pi_\theta^{\rm req}(q^*\mid o)\\
&+w_a\log\widetilde\pi_\theta^{\rm act}(a^*\mid o,q^*)\big].
\end{aligned}
\end{equation}
BC updates the actor; its saved critic remains fixed and external assessment uses executed events. The MAPPO and BC cohorts therefore retain separate checkpoint and action-interface identities.

GRPO's group comprises sampled candidate completions used to form a reward-relative training baseline~\cite{shao2024deepseekmath}. MAPPO's residents instead interact through state transitions, leases, ownership and timing. This choice matches centralized training to the recorded interacting-resident RL setting; the BC cohorts provide an alternative learned executor. SceneTeract combines semantic planning and geometric feasibility verification and additionally uses GRPO for feasibility prediction~\cite{maillard2026sceneteract}. TEAM-GRPO groups complete joint-household trajectory replicas for relative-return estimation, defining a different estimator over the same interacting-agent setting. Each declared executor is assessed through the same household-use functional $\mathcal Q$; outcomes retain their executor identity.



==> supplement_sections/c_dynamic.tex <==
\section{Resident Model and Event Semantics}
\label{app:dynamic_model}\label{app:learned_execution}\label{app:operational_model}\label{app:learning_details}
\subsection{Persistent state and actions}
The shared state contains time, positions, object anchors/owners, open states, pending jobs, leases, released requests and credited needs. Ready residents select requests and actions; scheduled completions update the persistent world. The actor observes logical state. Variable-duration commitments follow the semi-Markov view of temporal abstraction~\cite{sutton1999options}, with durations determined by modeled actions.

The daily interface has 258 actions: 32 object-indexed choices for NAV, OPEN, CLOSE, PICK, PLACE, USE, OFFER and ACCEPT, plus WAIT and sustained ACTIVITY. State-dependent masks restrict policy support~\cite{mask2022} through affordances and immediate eligibility. NAV uses profile-specific graphs; PICK/PLACE update ownership/support; sustained activities advance requests. Capacity-one resources use leases. Eligible actions can still loop without completing needs.

For resident $i$, the frozen policy factorizes as
\begin{equation}
\pi_\theta(q_i,a_i\mid o_i)=\pi_\theta^{\rm req}(q_i\mid o_i)\,
\widetilde\pi_\theta^{\rm act}(a_i\mid o_i,q_i).
\end{equation}
Both furnishings use identical weights and argmax decoding. Requests and actions are learned; temporal controllers remain separate. Unselected original needs remain in the evaluator.

\input{supplement_sections/c_architecture_learning}

\subsection{Matched execution and independent readout}
\label{app:criterion-algorithms}
Algorithm~2 states the execution/readout boundary. A fixed decoder acts on matched original needs; replay reconstructs actual outcomes before costs are compared. Unfinished obligations remain visible.

\begin{table*}[t]\centering\small
\begin{tabularx}{\textwidth}{@{}rY@{}}\toprule
\multicolumn{2}{@{}l}{\textbf{Algorithm 2. Matched household execution and independent readout}}\\\midrule
\textbf{Input}&Layouts $(\mathcal{L}_A,\mathcal{L}_B)$; household $H$, original needs $\xi$, frozen actor $\pi_\theta$ and execution contract.\\
\textbf{Output}&Verified need records, personal burdens, interactions and supported pairwise comparison.\\\midrule
1&Validate matched needs, profiles, schedules, decoding and semantics; retain identical physical starts for furnishing edits and admitted starts for cross-home comparisons.\\
2&\textbf{for each} layout $\mathcal{L}\in\{\mathcal{L}_A,\mathcal{L}_B\}$ \textbf{do}\\
3&\quad Initialize persistent state $x_0$ and retain every original need in the evaluator.\\
4&\quad \textbf{while} events or original needs remain, within the declared horizon and action budget \textbf{do}\\
5&\qquad For each ready resident $i$, select $q_i=\operatorname{Decode}(\pi^{\mathrm{req}}_\theta)$ and $a_i=\operatorname{Decode}(\widetilde\pi^{\mathrm{act}}_\theta(\cdot\mid q_i))$ with fixed decoding.\\
6&\qquad Schedule admissible actions; commit the earliest completion and update shared resources, ownership and time.\\
7&\quad Independently replay the resulting events and reconstruct each resident's original-need outcomes and costs.\\
8&\textbf{if} both alternatives fulfill the complete matched need set, compare their household and personal burdens.\\
9&\textbf{else} retain incomplete, certified-adverse and unresolved outcomes without interpreting early abandonment as low cost.\\
10&\textbf{return} matched outcomes and evidence using the external assessment functional.\\\bottomrule
\end{tabularx}
\end{table*}

\input{supplement_sections/c_mappo_update}

\subsection{Behavioral cloning and competence}
For the BC objective defined above, constructive demonstrations supply the training targets. The whole-home actor descends from the rich-assessment BC checkpoint through daily balanced and event-uniform BC stages. Earlier MAPPO cohorts remain separate experiments (Table~\ref{tab:learning-cohorts}).

Daily actors clone admitted constructive demonstrations using weighted masked request/action cross-entropies. Uniform and skill-balanced variants change row/action weights. The kitchen comparison freezes three separately trained actors after six passes: uniform seeds 4101/4102 and balanced seed 4103.

Actions alter subsequent observations, making closed-loop performance dependent on the policy-induced state distribution~\cite{ross2011dagger}. Normalization placement also affects Transformer optimization~\cite{xiong2020layernorm}. We assess competence through executed original needs and recomputed burden. Appendix~F separates fixed-weight request/action interventions from weight-changing adaptation and its retention check.

\paragraph{Policy learning and external assessment.}
PPO optimizes a clipped surrogate~\cite{ppo2017}; GAE trades bias against variance in advantage estimation~\cite{gae2016}. Independent PPO uses local value estimates~\cite{ippo2020}; COMA assigns credit through counterfactual baselines~\cite{foerster2018coma}; QMIX factorizes team values monotonically~\cite{rashid2018qmix}. These optimize return; our resident burdens are external measurements. The MAPPO/GRPO distinction is detailed in Section~\ref{app:architecture-learning}.

\subsection{Clock, waiting and original needs}
The engine processes the earliest pending completion, rounding positive sub-microsecond activity residuals upward to one microsecond. This corrects a legacy defect that could prolong a five-second activity until an unrelated request. Main-paper daily comparisons use the corrected clock; independent replay checks actions and times. Historical Appendix~F diagnostics retain their protocols.

Primary burden includes instrumental actions, invalid-attempt time and forced waiting; desired eating, rest and work are excluded. Voluntary waiting enters a separate sensitivity comparison. Unfinished released needs stay in the denominator; matched costs require all original needs to complete.

\paragraph{Reproducibility.}
Section~\ref{app:policy_choice} specifies the matched comparison contract; Algorithm~2 defines replay and readout. Scene, execution, need and action counts retain separate denominators; research records preserve run histories.



==> supplement_sections/c_mappo_update.tex <==
\subsection{Centralized training for the recorded MAPPO branch}
Algorithm~3 makes the recorded native MAPPO update explicit. Ready residents contribute separate action rows but share an event-level advantage from the current joint-state critic. The time-aware recursion uses $\gamma_n=\gamma^{\Delta t_n/u}$ and $\lambda_n=\lambda^{\Delta t_n/u}$, where $u$ is the declared time unit. This is the finite-TRAIN-epoch branch studied below; the request-conditioned daily/family BC branch retains its separate cross-entropy objective.
\begin{table*}[t]\centering\small
\begin{tabularx}{\textwidth}{@{}rY@{}}\toprule
\multicolumn{2}{@{}l}{\textbf{Algorithm 3. Event-based MAPPO with a current joint-state critic}}\\\midrule
\textbf{Input}&Shared actor $\pi_\theta$, centralized critic $V_\phi$, admitted training cases, rollout length, PPO budget, time unit $u$.\\
\textbf{Output}&Updated actor and critic; checkpoint preserving optimizer, collector and random state.\\\midrule
1&Initialize training worlds and a frozen actor anchor $\pi_{\rm ref}$; retain their original exogenous cases.\\
2&\textbf{while} admitted training cases remain \textbf{do}\\
3&\quad Collect a rollout: for each event, record the current joint state $s_n$ and $V_\phi(s_n)$ before acting.\\
4&\quad Each ready resident samples a masked action; record its old log probability and execute the joint dispatch.\\
5&\quad Record reward, elapsed time $\Delta t_n$, terminal flag and final next-state value before any reset.\\
6&\quad Compute backwards $\delta_n=r_n+\gamma_n(1-d_n)V_{n+1}-V_n$ and $A_n=\delta_n+\gamma_n\lambda_n(1-e_n)A_{n+1}$.\\
7&\quad Map event advantages to resident rows and normalize once over the rollout to obtain $\widehat A_{n,i}$ for the actor.\\
8&\quad For each PPO epoch and minibatch, minimize the negative clipped surrogate, minus entropy, plus the configured $\mathrm{KL}(\pi_\theta\Vert\pi_{\rm ref})$ anchor.\\
9&\quad Separately update $V_\phi$ by mean squared error to $A_n+V_n$ using the original, unnormalized $A_n$ over valid world events.\\
10&\quad Preserve the distinct actor/critic optimizer states and the exact continuing world and scheduler state.\\
11&\textbf{return} the trained checkpoint; evaluate household needs with the separate executed-event readout.\\\bottomrule
\end{tabularx}
\end{table*}
Here $d_n$ marks an actual terminal and $e_n$ an episode boundary: continuing cuts retain their bootstrap, while resets end the bootstrap chain. Entropy and anchor terms regularize training; the external functional measures furnishing quality.


==> supplement_sections/d_paired_quality.tex <==
\section{Matched Evaluation and Interpretation}
\label{app:resident_suitability}\label{app:human_protocol}\label{app:ablation_matrix}\label{app:complementarity_proof}
\subsection{Frozen pairing and scoring}
\label{app:policy_choice}\label{app:quality_interpretation}\label{app:dynamic_understanding}
Same-home furnishing comparisons fix the envelope, inventory and physical starts while changing the declared furniture placement or orientation. Cross-home comparisons instead match household, semantic needs and calendar through admitted task bindings and starts in each home. Both fix policy weights, decoding and cost rules. We report completion, unresolved coverage and operational burden separately. Repeated request realizations are grouped within their source family. We report source-family counts and repeated draws separately for uncertainty-aware interpretation of few-run RL estimates~\cite{agarwal2021}.

\subsection{Original needs and observed burdens}
For scored intervals $I_{im}$, resident $i$'s path $\ell_i$ sums committed NAV distances. Active time is skill occupancy intersected with those intervals; waiting follows the declared idle/WAIT/BLOCKED accounting. A shared handoff is one committed event but occupies both participants. Pre-request idle time is excluded where the scoring interval starts at request release. Missed semantic demands and missed primitive predicates retain different denominators.

Every unmet demand is classified as independently verified unmet or unresolved. Cost attribution uses the declared reference or proof assumptions. A certificate based on a fixed navigation graph is scoped to that graph. Cause-specific resource waiting is represented separately from total observed waiting. We report forced and voluntary waiting separately and test the sensitivity of furnishing order to including both.

\subsection{Measured household contrasts}
\label{app:household-main-protocol}
The contrasts below use the pairing contract in Section~\ref{app:policy_choice}, with fixed event semantics. Request randomness and policy-action randomness have separate roles.

\paragraph{Interaction cost.}
For unchanged personal needs, the additive joint-versus-solo contrast is
\begin{equation}
I(\mathcal{L},H)=C_\Sigma^{\mathrm{joint}}(\mathcal{L},H)-C_A^{\mathrm{solo}}(\mathcal{L},p_A)-C_B^{\mathrm{solo}}(\mathcal{L},p_B).
\end{equation}
Joint-only tasks are excluded from this estimand. The reference experiment crosses shared/private logical resources with request offsets, mobility profiles and furnishing variants. The private-resource control yields zero interaction, while shared resources give positive cost for synchronous requests. This control identifies the contribution of resource coupling. Helping uses a separate matched intervention with unchanged personal obligations.

\paragraph{Profile-dependent furnishing order.}
For furnishings $\mathcal{L}_A,\mathcal{L}_B$, define $\Delta_H=C_\Sigma(\mathcal{L}_A,H)-C_\Sigma(\mathcal{L}_B,H)$. A reversal has opposite signs under two household profiles and requires complete original-need fulfillment in every compared condition. The measured mobility intervention changes resident B's capability parameters while preserving request contents. The house-00685 contrast is reported separately for the initial request draw and three additional timing realizations.

\paragraph{Synchronization and temporal controls.}
Holding request contents fixed, we measure
\begin{equation}
\delta=\Delta_H^{\mathrm{sync}}-\Delta_H^{\mathrm{offset}}.
\end{equation}
The reported comparisons use a 180-second request offset, profile-weighted routes, request-priority search and finite start-delay search. The temporal controls have full information about the modeled day. Their different waiting components explain why removing forced waiting can lower primary burden while increasing voluntary delay. Algorithms are compared under the same original needs, with completion coverage reported beside cost.

\subsection{Open questions for household-conditioned assessment}
\label{app:open-questions}
\textbf{Executor sensitivity.} Which furnishing orders remain stable across independently competent executors? Matched needs and completion support comparisons of scheduling and personal costs under a common external functional.

\textbf{Routine coverage.} Which additional needs make an otherwise unused furnishing change observable? A coverage map from household activities to affected objects and routes can guide finite, interpretable scenario selection.

\textbf{Household calibration.} How should numerical capabilities and the declared preference rubric be calibrated for a target household? Separating physical parameters from preference weights allows each source of evidence to be assessed directly.

\textbf{Physical co-presence.} How do continuous body motion, mutual passage and access envelopes change conclusions based on logical resource sharing? This extends the shared-state formulation from timed ownership and cooperation to simultaneous use of physical space.

\subsection{Source-family construction}
All 12,000 original source identities are accounted for: 11,994 adapted houses and six unadapted entries. The input-capability audit checks adapted payload hashes and excludes declared geometry/source/contour families crossing official splits, as well as unsupported metadata. Eight development families are selected from the original validation split by an immutable hash ordering, requiring at least two reusable tableware nodes and a nonportable dining table. Five pass the subsequent geometry, common-start and task-binding checks used in the reported household experiment. These rules define its restricted task population.


==> supplement_sections/e_data.tex <==
\section{Datasets, Splits and Exclusions}
\label{app:construction_audit}\label{app:whole_apartment_semantics}
\subsection{Rich furnishing cohort}
\label{app:rich_full_audit}
The rich source/geometry/alias review admits 7,704 parent houses from the original official training split. Parent and alias partitions were frozen before outcomes: 6,224 training, 701 development and 779 locked test. Two households and six recipes per parent give 92,448 fixed conditions: 74,688/8,412/9,348 by partition. The original official validation and test houses remain reserved. Collection and independent source/replay/semantic/cost checks reconcile the fixed evaluation population; dwelling outcomes are reported separately.
\begin{table}[t]\centering\small
\caption{Rich training reference verdicts, retaining every fixed condition and unknown.}
\begin{tabular}{@{}lrrr@{}}\toprule
Branch&Positive&Negative&Unknown\\\midrule
Static 0&41,244&21,782&11,662\\
Dynamic&228&5,261&69,199\\
Combined&228&27,043&47,417\\\bottomrule
\end{tabular}\end{table}
The training set contains 5,583 observed episode payloads: 228 positive, 5,261 negative and 94 unknown. Their original input/target, competence, cost and leakage checks pass; 1,834,795 actor rows are eligible constructive demonstrations. Observed behavior categories are 728 competent-full, 3,798 best-attainable partial and 1,057 non-demonstration episodes. Imitation targets include demonstrated actions only.

The full training-set semantic denominator is 8,445,192: 347,086 met, 199,465 verified unmet and 7,898,641 unknown. Observed episodes contain 563,199 semantic demands; all remaining conditions retain their recorded evaluation status. Across all partitions, 6,953 constructor/restore records and 6,949 indexed episode payloads are distinct from successful weeks. 

Strict matching uses source house, household, original requirements/physical-start context, criteria, world seed, scenario and source version. Dynamic yields 21 positive--negative pairs in 13 contexts/ten houses, versus 363 Combined pairs in 145 contexts/118 houses, among 186,720 possible within-context training pairs. The larger Combined count may follow Static 0. These metadata describe the reference cohort; neural discrimination is evaluated through actor executions.


==> supplement_sections/f_bc_progression.tex <==
\paragraph{Historical checkpoint progression.}
Figure~\ref{fig:training-competence} organizes the existing daily-pilot and expansion evaluations by training progress. These historical checkpoints are separate from the current family actors.

\begin{figure*}[t]\centering
\includegraphics[width=.94\textwidth]{figures/cohabit_training_competence.pdf}
\caption{\textbf{Demonstration fitting and retained execution are distinct measurements.} (a) Completed daily sessions at the two evaluated cloning checkpoints, for all three paired seeds. (b) Retained completion after the demonstration set expands, for the two shared-parent seed pairs. Each observation evaluates the same 18 sessions and 96 original needs under its declared historical execution contract. Zero in (b) denotes the accepted daily parent. Lines connect the measured checkpoints. Seeds replicate fine-tuning on the same exposed scenes. No population confidence interval is implied.}
\label{fig:training-competence}
\end{figure*}


==> supplement_sections/f_complex_trajectories.tex <==
\subsection{Multi-room routines and joint execution}
\label{app:complex_trajectories}
The following saved executions show how repeated activities use a furnished home over time. The first example follows one resident across several rooms; the next two distinguish simultaneous personal routines from an actual transfer between residents. Each example retains its original agenda and model, so their goal counts and distances are read within the corresponding scenario.

\begin{figure*}[t]\centering
\includegraphics[width=.86\textwidth]{figures/complex_week_trajectory.pdf}
\caption{\textbf{A full week of routes through a furnished home.} The saved PPO execution in house 00277 completes 21 stages and all 90 original goal conditions. Its 109 NAV actions cover 42 distinct directed endpoint pairs and total 1033.35\,m; recorded stops occupy five of six rooms. Colors denote the seven days, arrows give travel direction, and the circle and square mark the initial and final positions. Repeated routes overlap at their true coordinates. This single-resident example illustrates spatial coverage and repetition of the prescribed routine.}
\label{fig:complex-week-trajectory}
\end{figure*}

All routes are reconstructed from saved committed actions using the declared profile-specific free-space graph. Original floor and furniture geometry, door openings, endpoints, per-action distances and total distance are checked. The polylines represent admissible static NAV paths. These historical illustrative executions are separate from the daily-policy experiments in the main paper.

\begin{figure*}[t]\centering
\includegraphics[width=\textwidth]{figures/joint_trajectory_examples.pdf}
\caption{\textbf{Two residents: concurrent routes and a repeated object relay.} Blue denotes resident 1 and dashed pink resident 2; circles and squares show starts and finishes. (a) In house 00123, both residents move between activity locations while completing all 18 goal conditions of the one-day agenda. Seven NAV actions total 83.85\,m. This is parallel execution, with no handoff. (b) In house 00897, the seven-day relay completes 126/126 goal conditions and records 21 successful handoffs. Resident 1 remains at the transfer location while resident 2 makes 22 journeys, totaling 227.70\,m. Repeated traversals share their plotted paths. (c) The first relay, directly from committed event times: resident 1 picks up the item; resident 2 navigates to the partner; both participate in the same 1.5-second handoff; resident 2 then travels to the destination and places the item. The full chain finishes 22.5 seconds after release. Gold bars mark a single shared event.}
\label{fig:joint-trajectory-examples}
\end{figure*}

The two panels use the same historical MAPPO checkpoint but different homes and agendas. They illustrate verified behavior under their recorded execution conditions. In particular, the stationary partner in the relay participates in every transfer: a resident can contribute to joint completion without accumulating a long route. The model attributes physical access to declared geometry and contention to logical-resource events; route plots show the spatial component.


==> supplement_sections/f_evidence.tex <==
\section{Additional Household Results and Examples}
\label{app:behavioral_cloning}\label{app:policy_diagnostics}\label{app:frozen-temporal}
\subsection{Shared-resource and temporal controls}
The corrected-clock reference experiment contains $5\times2\times2\times8\times3\times2=960$ executions: families, furnishings, mobility profiles, request offsets, joint/solo occupancy and shared/private resources. Every execution fulfills its original needs. Independent replay verifies the committed decisions and recomputes the readout. The private-resource control namespaces non-actor leases by resident, preserving personal requests, starts and geometry.
\begin{figure*}[t]\centering
\includegraphics[width=.94\textwidth]{figures/interaction_gap_corrected.pdf}
\caption{Interaction cost $I(g)$ across every admitted family, furnishing and mobility profile. Private resources give zero interaction. Shared resources produce cost at overlapping request times, which disappears as requests separate. Curves are individual development observations.}
\label{fig:interaction-gap}\end{figure*}

\begin{figure}[t]\centering
\includegraphics[viewport=0 0 252 165,clip,width=\linewidth]{figures/h23_reference_pilot.pdf}
\caption{\textbf{Furnishing-order control on the same reference cohort.} Synchronous A--B costs under matched speed and slower resident B reuse the corrected-clock executions in Figure~\ref{fig:interaction-gap}. Positive A--B favors B.}
\label{fig:h23-reference}\end{figure}

The priority controller enumerates six prerequisite-compatible orders per resident. A separate delay controller evaluates fixed offsets of 0,30,60,90,120,150,180 and 240 seconds, with 15 joint and eight solo candidate schedules per condition. Candidate selection prioritizes complete needs, then burden, with microsecond-precision and deterministic ties. These finite controllers know the modeled day in advance.

\begin{table}[t]\centering\small\setlength{\tabcolsep}{3pt}
\caption{Frozen comparison eligibility. Each method has 120 executions and 640 original needs. An interaction requires complete joint and both solo executions.}
\label{tab:frozen-eligibility}
\begin{tabular}{@{}lrrr@{}}\toprule
Method & Complete & Needs met & $I$ eligible\\\midrule
Uniform 4101 & 88/120 & 484/640 & 24/40\\
Uniform 4102 & 56/120 & 360/640 & 8/40\\
Balanced 4103 & 32/120 & 256/640 & \textbf{0/40}\\
Priority search & \textbf{120/120} & \textbf{640/640} & \textbf{40/40}\\
Delay search & \textbf{120/120} & \textbf{640/640} & \textbf{40/40}\\\bottomrule
\end{tabular}\end{table}
Balanced cloning has zero eligible interaction comparisons, so its contrast is recorded as unavailable. This comparison measures the combined change of seed and weighting.

\begin{figure*}[t]\centering
\includegraphics[width=.94\textwidth]{figures/temporal_wait_decomposition.pdf}
\caption{Why schedule selection changes burden. Each point averages four synchronous joint furnishing/profile conditions in one family. Voluntary waiting is shown separately from instrumental cost and witnessed forced waiting.}
\end{figure*}
On the twenty synchronous joint conditions, mean instrumental time is 24.52\,s for both temporal controls. Priority search adds 463.00\,s of forced waiting; delay search instead adds 242.85\,s of voluntary waiting and zero forced waiting. Thus primary burden is 487.53 versus 24.52\,s, while including voluntary waiting gives 267.37\,s for delay search. This identifies the role of scheduling and the selected cost definition.

An initial-input route proxy sums start-to-item, item-to-serving-surface and surface-to-seat graph distances, divides by resident speed, and adds the configured three seconds per resident for PICK and PLACE. Across all forty joint inputs it matches delay-search primary cost to within $4.3\times10^{-14}$\,s. After forced waiting is removed, the primary cost of this kitchen task family is explained by routes and fixed manipulation costs.

\subsection{Assistance and waiting attribution}
The matched intervention preserves A's work and B's delivery/consumption needs, permitting either A or B to deliver B's object. Reactive execution reverses A/B order in four of five families. Finite scheduling removes those primary-cost reversals. When voluntary waiting is included in both schedule selection and the readout, families 00359 and 00967 retain reversals, with no-help/help contrasts $+3.00/-11.00$ and $-8.25/+0.75$\,s. All sixty executions and 120 needs per control are verified.
\begin{figure*}[t]\centering
\includegraphics[width=.94\textwidth]{figures/help_wait_sensitivity.pdf}
\caption{Assistance-conditioned furnishing order under different controllers and waiting definitions. The waiting-inclusive controller is selected using the same quantity that is reported. Desired activity is excluded throughout. Points are individual development-family observations.}
\label{fig:help-wait-sensitivity}\end{figure*}
\begin{table}[t]\centering\small
\caption{Mean joint-time components over ten furnishings per row. $C$ includes instrumental and forced-wait time; $V$ is voluntary waiting. All original needs are fulfilled. Components are rounded independently.}
\label{tab:help-wait-components}
\begin{tabular}{@{}llrrr@{}}\toprule
Controller & Help & $C$ & $V$ & $C+V$\\\midrule
Reactive & Off &261.92&0.00&261.92\\
Reactive & On &252.70&9.47&262.17\\
Min. $C$ & Off &13.70&313.86&327.56\\
Min. $C$ & On &14.28&601.97&616.24\\
Min. $C+V$ & Off &118.61&133.63&252.24\\
Min. $C+V$ & On &252.70&9.47&262.17\\\bottomrule
\end{tabular}\end{table}
The apparent primary-cost benefit can exchange forced waiting for longer voluntary delay. This explains why the ranking changes with the accounting rule. A separate frequency intervention doubles B's kitchen episodes; both controllers fulfill all 800 original needs across 120 conditions, with unchanged instrumental costs. The object remains on its serving surface after the first delivery, and subsequent desired consumption is excluded from burden, explaining this null frequency effect.

\subsection{Profile contrast across request-time draws}
Uniform actor 4101 is frozen after its selection by development completion. Three additional request-time draws retain all five families, both furnishings and mobility profiles, and both offsets, giving forty joint conditions and 320 needs per draw. Each draw yields 32/40 complete executions and 260/320 fulfilled needs. Delay search completes all 120 conditions and 960 needs across the three draws.
\begin{figure*}[t]\centering
\includegraphics[width=.94\textwidth]{figures/learned_profile_replication.pdf}
\caption{The same frozen actor in house 00685 under the original and three additional request-time draws. Positive A--B favors B. The synchronous profile-conditioned reversal repeats; the asynchronous contrast varies. Lines connect individual realizations.}
\label{fig:learned-profile-replication}\end{figure*}
The synchronous A--B contrasts are $+3.75,+3.75,+3.75$\,s for matched speed and $-1.25,-6.25,-1.25$\,s for slower B. Every condition entering these contrasts fulfills its original needs. The synchronous reversal persists after subtracting recorded invalid-attempt time. This is a repeated local effect of the frozen behavior; the matched temporal controller retains the same furnishing order across profiles.

\subsection{Interpreting execution and retention effects}
On the same forty conditions, replacing request selection alone leaves completion at 32/40. Replacing primitive execution gives 36/40 and eliminates the action-limit cuts. Recorded failures include repeated valid NAV to the current node and persistent idle-request selection. The guards below test those two mechanisms with unchanged weights, needs, geometry and deadlines.
\begin{table}[t]\centering\small
\caption{Matched execution interventions. All rows retain forty conditions and 320 needs. Guards change inference rules; reference-action rows diagnose execution.}
\begin{tabular}{@{}lrr@{}}\toprule
Variant & Complete & Needs met\\\midrule
Original policy &32/40&260/320\\
Reference requests &32/40&260/320\\
Reference actions &36/40&304/320\\
Navigation guard &34/40&298/320\\
Request guard &32/40&260/320\\
Both guards &\textbf{37/40}&\textbf{310/320}\\
Reference actions + request guard &\textbf{40/40}&\textbf{320/320}\\\bottomrule
\end{tabular}\end{table}
Both guards improve completion to 37/40, while reference actions with the request guard complete all forty conditions. The former is a measured execution improvement under changed inference; suppressing idle requests also changes willingness to act, so competence and behavioral interpretation remain separate.

\label{sec:revision-audit}\label{sec:short-repair-pilot}
A separate one-epoch BC adaptation of uniform actor 4101 reduces learning rate and increases PICK/PLACE weight over the same 8,450 admitted rows (34 updates). On the eighteen matched retention conditions, completion falls from 18/18 to 15/18 and fulfilled needs from 96/96 to 84/96; valid PICK and PLACE commits each fall from 27 to 24. The adapted actor completes 43/48 expanded conditions and 248/256 needs. Independent replay verifies all eighty-four executions. This is an adverse retention effect on matched inputs; learning rate and weighting changed together, so neither is identified as its sole cause. The expanded set measures a separate population; the matched retention result records the regression.


\subsection{Family calendars and comparison coverage}
Two adults and a child execute three whole-home scenarios under six numerical profiles, two request draws and synchronous or shifted calendars. Each actor has 144 executions with 3,024 original needs. Two initial actors complete 120 and 108 executions and each admits 54 of 72 matched comparison contexts. Both complete all synchronous cases; incomplete shifted traces concentrate on assistance coordination. In the matched-update comparison, synchronous-only controls complete 108 and 114 executions, whereas both diverse-calendar actors complete all 144 and all needs, expanding context coverage from 54 to 72. Demonstration diversity and size change together. In every diverse-calendar comparison, all three individual costs favor B. In the birthday example in the main paper, B reduces adult/child latency by approximately 76, 58 and 79 need-seconds.

\paragraph{Independent units in the main family table.}
Development uses two homes (00650 and 00967); unfitted transfer uses two additional TRAIN-pool homes (06417 and 08887). Each calendar contains $2\times3\times6\times2=72$ executions across homes, routines, profiles and request draws. The last column counts $1\times3\times6\times2\times2=72$ contexts of one fixed home-pair across two calendars. Parenthesized repetitions use paired training seeds 7201 and 7202; the request draws are 74501 and 74502. These are controlled comparisons on fixed homes. We report exact completion counts for each seed on 72 repeated contexts of the same apartment pair. With two homes, a house-cluster bootstrap has at most three distinct resampled means and collapses for all-complete cells; uncertainty on new homes requires additional source geometries.

\input{supplement_sections/f_learning_cohorts}
\input{supplement_sections/f_retained_results}

\input{supplement_sections/f_execution_readiness}

\input{supplement_sections/f_whole_home}
\input{supplement_sections/f_complex_trajectories}
\input{supplement_sections/f_trajectory_examples}
\input{supplement_sections/f_reference_examples}
\subsection{An additional controlled furnishing intervention}
\label{app:expanded_paired_comparison}\label{app:competence_census}
The retained house-01869 example uses the earlier fixed-agenda policy and 105 original demands per furnishing. Its side-table group moves rigidly by 0.60\,m. The source-bound panels below distinguish achieved, independently certified-unmet and unresolved needs; efficiency comparisons require complete execution.
\begin{figure*}[t]\centering
\includegraphics[width=\textwidth]{figures/matched_furnishing_pair.pdf}
\caption{\textbf{Actual furnishing intervention within the controlled matrix.} House 01869 keeps the same residents, starts and 105 demands; B moves a side table and its supported items $+0.60$\,m in the floor plane. MAPPO meets 56/105 versus 42/105 demands. Bars retain certified-unmet and unresolved needs. A remains unknown; B is negative only through a scoped model certificate. This selected training example illustrates a reference-conditioned contrast.}
\label{fig:frozen-pair}
\end{figure*}





==> supplement_sections/f_execution_readiness.tex <==
\subsection{Admissibility and routine composition}
\label{app:execution-readiness}
Six development cases hold actor 4101's weights, geometry, households and original needs fixed across interfaces. The cohort spans two homes and one calendar. Interfaces developed on this cohort constrain current-state choices without teacher replacement, defining distinct executed policies.

\begin{table}[tb]\centering\small
\caption{\textbf{Matched admissibility interventions.} Six cases and 106 original needs per row; all executions independently replayed, without weight updates.}
\label{tab:whole-home-readiness}
\begin{tabular}{@{}lrr@{}}\toprule
Decision interface & Complete & Needs met\\\midrule
Original affordances &0/6&8/106\\
Activity readiness &0/6&33/106\\
Suppress idle request &0/6&11/106\\
Activity + idle control &0/6&33/106\\
Physical readiness &\textbf{2/6}&\textbf{71/106}\\\bottomrule
\end{tabular}\end{table}
Idle is suppressed only with an eligible need. Physical readiness adds manipulation preconditions to activity readiness, preserving navigation, transfer, waiting and request selection. It completes the illustrated home's independent-day and shared-evening joint routines; the paired home reaches the kitchen stage but leaves later needs unmet. Both contrasts remain horizon-censored policy outcomes, separating local admissibility from complete-routine assessment.

\begin{figure}[tb]\centering
\includegraphics[width=\linewidth]{figures/whole_home_readiness.pdf}
\caption{\textbf{Admissibility exposes joint execution.} The shared-evening example uses fixed actor weights and original needs. Physical readiness completes the joint routine, including a shared meal and conversation. Curves reconstruct verified committed navigation; rings mark coincident start/end positions.}
\label{fig:whole-home-readiness}
\end{figure}


==> supplement_sections/f_learning_cohorts.tex <==
\subsection{Learning branches and recorded training progress}
\label{app:learning-cohorts}
Table~\ref{tab:learning-cohorts} resolves training identity before interpreting an executor's results. MAPPO was trained and evaluated in three earlier branches; the daily and family furnishing comparisons use BC-trained actors. The accepted checkpoint and training record identify each actor's algorithm.

\begin{table*}[t]\centering\small
\caption{Learning provenance of the reported resident cohorts. Source hashes and logs accompany the materials. Checkpoint identity includes interface, data and evaluation contract as well as seed.}
\label{tab:learning-cohorts}
\begin{tabularx}{\textwidth}{@{}p{.19\textwidth}p{.19\textwidth}p{.21\textwidth}Y@{}}\toprule
Cohort & Training & Checkpoint or trace & Evidence supported\\\midrule
Fixed agendas & MAPPO & Seed 103, update 406 & One-day parallel routine (18/18 goals); seven-day relay (126/126, 21 handoffs). Verified trajectory examples under fixed agendas.\\
Native finite-TRAIN & MAPPO & Seeds 302--304; 58,043 training cases per seed & Iteration-level training progress in the native training runtime.\\
Rich optimization & BC warm-up, then MAPPO & Seeds 201--205; privileged and route-hidden & Ten iteration traces describe optimization. The frozen comparison below uses its own fixed evaluation cohort.\\
Rich frozen comparison & BC predecessor versus MAPPO & Route-hidden seed 201, before/after RL & Matched need coverage and tie-adjusted ordering on 21 selected pairs, 32 TRAIN conditions and ten houses.\\
Daily and whole-home & Behavioral cloning & Daily seeds 4101--4103; whole-home 6101, update 512 & Corrected-clock household comparisons; whole-apartment and shared-50-pair executions use the declared fixed interface.\\
Family volume-changing & Offline behavioral cloning & Seeds 7201--7202; single/diverse, update 2,048 & Four actors; 28,506 versus 81,462 demonstration examples. Main-paper calendar comparison and initial transfer.\\
Family matched-volume & Offline behavioral cloning & Seeds 7201--7204; synchronous/diverse, update 2,048 & Eight paired-calendar actors; fixed 27,158 examples per condition; temporal and geometric transfer tests retain their own splits.\\\bottomrule
\end{tabularx}
\end{table*}

\paragraph{Iteration-level MAPPO observations.}
Figures~\ref{fig:training-rich-mappo} and~\ref{fig:training-native-mappo} retain the separate five-seed rich-assessment and three-seed native cohorts. Each plotted value comes from an actual logged update, with minibatch metrics aggregated within that update. Recorded endpoints differ across runs. These curves expose optimization and training progress; verified original-need outcomes below provide the behavioral evidence.

\begin{figure*}[t]\centering
\includegraphics[width=.94\textwidth]{figures/rich_mappo_iteration_traces.pdf}
\caption{\textbf{Recorded MAPPO optimization across five initializations.} Privileged and route-hidden observations are shown separately, with actual update coordinates and per-update minibatch means. Curves stop at the corresponding recorded endpoints. Policy loss uses a symmetric logarithmic scale; entropy uses a linear scale. Both statistics describe policy optimization; held-out execution measures household competence.}
\label{fig:training-rich-mappo}
\end{figure*}

\begin{figure*}[t]\centering
\includegraphics[width=.94\textwidth]{figures/native_mappo_iteration_traces.pdf}
\caption{\textbf{Native-runtime MAPPO iterations for seeds 302--304.} This cohort is separate from the rich-assessment branch above. Left: recorded success in the latest 128 completed TRAIN episodes. Right: policy loss at actual logged updates. Rolling training windows measure progress on changing training cases.}
\label{fig:training-native-mappo}
\end{figure*}


==> supplement_sections/f_reference_examples.tex <==

\subsection{Reference-execution examples across apartments and households}
\label{app:desktop_reference_gallery}
These four post-hoc illustrations reuse the archived reference trajectories from the earlier 24-condition CPU pilot: 16 modeled weeks, six positive, ten negative and eight unknown outcomes. Its visit agenda and 150/75\,m budgets differ from the rich 900\,m study. Original polygons, object identities, rigid edits, goals, physical starts and readouts are retained; no new NAV, simulated episode or neural call produced these figures. Bounding-box footprints and the fixed 2.5D graph define the spatial approximation used in these simulated activities.

Pilot static approval checks for added overlap; broader ergonomic criteria have their own assessment. G1/G2 are saved targets, S1/S2 are starts, and bars are one model metre. No continuous paths are reconstructed. Selected examples explain mechanisms under their recorded conditions.
\begin{figure*}[t]\centering
\includegraphics[width=.90\textwidth]{figures/reference_example_1.pdf}
\caption{\textbf{Different apartments, same declared household.} Both standard/fast residents meet 21/21 visit requirements. In 01110, paths 98.70/105.75\,m satisfy the 150/150\,m contract. In 01100, paths 155.40/166.50\,m exceed it, supporting a cost-negative operational assessment despite completion. Both pass the pilot's relative no-new-overlap condition. This comparison uses different apartments and a reference executor under the declared criteria.}
\label{fig:desktop_different_houses}
\end{figure*}


\begin{figure*}[t]\centering
\includegraphics[width=.90\textwidth]{figures/reference_example_2.pdf}
\caption{\textbf{Actual matched furnishing pair without a verdict flip.} In 01110 the saved dining-table/support group shifts by 0.50\,m along the source $x$ axis; envelope, household and visit requirements remain fixed. Orange marks edited geometry; dashed outlines show its old position. Paths rise from 98.70/105.75 to 113.40/121.50\,m, while all 21/21 visit requirements per resident and both 150\,m limits are satisfied. Both outcomes remain positive under this contract; the translation changes travel costs without changing the contract verdict.}
\label{fig:desktop_furnishing_pair}
\end{figure*}


\begin{figure*}[t]\centering
\includegraphics[width=.90\textwidth]{figures/reference_example_3.pdf}
\caption{\textbf{Same furnishing, different household contract.} R2 changes from fast to wide-clearance and its path limit changes from 150 to 75\,m. Under the saved fixed-graph access model, R2 meets 7/21 visits, with 14 verified unreachable visits at G2; R1 remains 21/21. R2 remains at its initial G1 node, completing the seven colocated visits with 0\,m travel; fourteen other required visits remain unreachable. The blocked-target annotation refers only to that stored graph certificate. Profile and budget change jointly under the fixed-graph access model; the resulting infeasibility verdict is scoped to that graph.}
\label{fig:desktop_household_change}
\end{figure*}


\begin{figure*}[t]\centering
\includegraphics[width=.90\textwidth]{figures/reference_example_4.pdf}
\caption{\textbf{Unknown retains its denominator.} Source 01110 has verified reference readouts; 02148 lacks a preserved valid physical-start binding for the attempted condition. Its source plan is displayed with the attempted execution recorded as unresolved. All 21 required visits per resident remain in the denominator; completion and distance retain unknown values. The unresolved source condition retains an unknown furnishing verdict.}
\label{fig:desktop_unknown}
\end{figure*}



==> supplement_sections/f_retained_results.tex <==



\subsection{Additional measured competence results}
\label{app:retained-diagnostics}
These historical studies separate execution competence from layout assessment. Rich actors use the earlier fixed-agenda, 257-action interface; the daily pilot predates the corrected-clock comparisons. Results are reported separately by execution contract.

\paragraph{Frozen comparisons and necessary bounds.}
Twenty-one reference-selected pairs reuse 32 training conditions in ten houses. Frozen BC, MAPPO and legal-mask control executions share exogenous draws and independent replay; learned decoding is FP32 masked argmax. Pair ordering gives half credit to ties:
\begin{center}\small\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lrr@{}}\toprule
Policy & Met / required & Pair ordering\\\midrule
BC predecessor &90/2,884&.524\\
Subsequent MAPPO &\textbf{1,204/2,884}&\textbf{.762}\\
Legal-mask control &0/2,884&.500\\\bottomrule
\end{tabular}\end{center}
All methods have 0 positive, 11 certificate-negative and 21 unresolved verdicts: better demand ordering adds no verified classification gain.

Across 228 reference-feasible training conditions, two rich actors meet 9,910 and 4,299 of 21,112 demands, with no verified positive. Among 15 additional adverse cases, NAV+agenda bounds certify ten; stronger necessary checks certify eleven, without rejecting any feasible case. Both dynamic readouts inherit those eleven negatives. Necessary conditions explain the verified classification coverage; remaining cases are unknown.

\paragraph{From demonstrated actions to closed-loop skills.}
The corpus contains 285,090 manipulation targets among 1,834,795 eligible rows, yet final actors request only NAV/WAIT in 439 executions. On 2,736 familiar manipulation states, seed-201 demonstrated-action agreement falls from 2,317 after BC to 333 after adaptation; seed~205 yields eleven. A retention snapshot matches 403/456 PICK targets but commits no valid PICK in 228 executions, fulfilling 392/21,112 demands. BC navigation agreement was already weak: 5/226 picked-goal and 10/142 handoff-goal states. These contrasts compare checkpoints together with their recorded training protocols.

On eighteen short-chain cases with three action draws, BC completes 2/54 and final retention 0/54; neither completes handoff or parallel delivery. These probes evaluate exposed houses under the legacy clock; corrected-clock daily actors form a separate cohort. A modeled cross-room handoff completes in 22.5\,s with resident distances 0/20.70\,m, providing a verified event-sequence example.

\paragraph{Cloning gains are local and can regress after expansion.}
Checkpoint identity includes the training protocol as well as the seed: the pilot checkpoints below differ from the later corrected-clock kitchen actors carrying the same seed integers. The earlier daily pilot shares one parent and eighteen familiar-house sessions (96 needs) across three paired seeds. After six passes:
\begin{center}\small\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrr@{}}\toprule
Seed & Balanced: complete; met & Uniform: complete; met\\\midrule
4101 &17/18; 95/96&0/18; 38/96\\
4102 &\textbf{18/18; 96/96}&12/18; 81/96\\
4103 &\textbf{18/18; 96/96}&10/18; 72/96\\\bottomrule
\end{tabular}\end{center}
Fresh balanced initialization completes 9/18 sessions and 33/96 needs. Expanding to 48 demonstrations reduces retained completion from 17/18 and 18/18 to 12/18 and 15/18 after six passes under both weightings. Expanded coverage and matched retention are assessed separately. These outcomes measure local learning on the exposed routines. The later daily corpus contains 8,450 eligible NAV, PICK, PLACE, WAIT and ACTIVITY rows.

\input{supplement_sections/f_bc_progression}


==> supplement_sections/f_training_traces.tex <==
\paragraph{Iteration-level family training observations.}
\label{app:training-observations}
Figure~\ref{fig:training-family-bc} shows the measured training loss for the eight matched-calendar family actors. Each condition has 27,158 admitted examples and a fixed budget of 2,048 accepted optimizer updates. The archive retains 39 unique minibatch observations across the eight runs: the first two accepted updates and available progress snapshots. The exact replay of update two is counted once. The final retained loss is at update 2,045; the accepted full checkpoint is at update 2,048. Only observed points are plotted, without smoothing, imputed updates or uncertainty bands. These losses measure demonstration fitting; independently audited routine execution establishes comparison competence.

\begin{figure*}[t]\centering
\includegraphics[width=\textwidth]{figures/family_bc_observed_iterations.pdf}
\caption{\textbf{Iteration-level BC observations for four paired initializations.} Markers show all 39 retained optimizer-update observations under single and diverse calendars; connecting segments guide the eye without reconstructing missing iterations. Both conditions use the same training budget, with different observation densities. Both axes are logarithmic. The last retained loss is at update 2,045; accepted final states are at update 2,048. Independent execution establishes comparison competence.}
\label{fig:training-family-bc}
\end{figure*}



==> supplement_sections/f_trajectory_examples.tex <==
\subsection{Recorded resident trajectories}
\label{app:trajectory_examples}
Figure~\ref{fig:recorded-trajectories} shows two seven-day executions in furnished house 00663: two residents and 126 original goals. These earlier fixed-agenda examples are separate from the daily-policy comparisons.

\begin{figure*}[t]\centering
\includegraphics[width=\textwidth]{figures/recorded_resident_trajectories.pdf}
\caption{\textbf{Read routes together with fulfilled needs.} In the same furnished home, MAPPO fulfills 126/126 goals and travels 175.95\,m; TEAM fulfills 7/126 and travels 13.95\,m, also repeating 497 zero-distance NAV actions. Blue/pink denote residents; circles/squares mark starts/finishes. Repeated traversals share a route. Efficiency is assessed jointly with original-need completion. The executions compare the recorded policy--training combinations.}
\label{fig:recorded-trajectories}
\end{figure*}

\paragraph{What the lines represent.}
Lines reconstruct committed NAV actions on shortest-grid routes, checking geometry, endpoints and distances within the navigation model. Both executions remain in one room; this agenda has single-room coverage. Coincident endpoints retain overlapping markers.

\subsection{Calendar diversity at equal demonstration volume}
Each arm uses 36 demonstrations, 27,158 resident/action/selector-matched examples and 2,048 updates. All 288 cases per actor are independently audited across four paired initializations (Table~\ref{tab:family-matched-volume}).
\begin{table*}[t]\centering\small
\caption{Shifted completion out of 72. S: synchronous training; D: diverse calendars. Bold: higher.}
\label{tab:family-matched-volume}
\begin{tabular}{@{}lcccc@{}}\toprule
Repeat & Development S & Development D & Unfitted S & Unfitted D\\\midrule
1 &36&\textbf{72}&36&\textbf{42}\\
2 &48&\textbf{72}&36&\textbf{72}\\
3 &54&\textbf{72}&60&\textbf{72}\\
4 &66&\textbf{72}&36&36\\\bottomrule
\end{tabular}
\end{table*}
Transfer discordances (diverse-only/control-only) are 24/18, 36/0, 12/0 and 0/0 across repeats. Both repeat~4 actors fail on home 06417 under either calendar: unfitted synchronous coverage is 36/72, versus 72/72 in the other repeats. Thus aggregate gains coexist with local regressions and a shared transfer failure. Action-limit stops and their incomplete pair comparisons retain an unresolved verdict. These results cover the inspected development and TRAIN inputs under numerical simulator profiles.



\input{supplement_sections/f_training_traces}


==> supplement_sections/f_whole_home.tex <==
\subsection{Comparing furnished homes through whole-apartment routines}
\label{app:whole-home-comparison}
Matched routines link rest, sink use, deliveries, work, meals and conversation. Admitted furniture and routes support timed resource reservations.

Reference and finite temporal controllers each fulfill all 1,976 needs in 108 independently replayed executions across three admitted development homes. Each controller yields 84 complete joint and 12 complete single-resident comparisons. Opposing resident costs occur in 14 reference and 20 temporal joint comparisons. Profiles are compared on common admitted homes.

Matched households and calendars retain completion and personal pending-need latency:
\begin{equation}
L_i=\sum_{r:\,i\in\mathcal B_r}\bigl(\min\{T_r,\tau\}-a_r\bigr),\qquad L_\Sigma=\sum_i L_i.
\end{equation}
The sum covers the original needs released by $\tau$ ($a_r\leq\tau$). Here $a_r$ is release time, $T_r$ is physical completion ($+\infty$ if unmet), $\tau$ is the common horizon, and $\mathcal B_r$ contains beneficiaries. Shared needs contribute to both residents. $L_\Sigma$ measures pending-need time (reported as $L_\Sigma$ in the route figure); earlier results retain their stated burden definition $C$.

\textbf{Scheduling control.} For synchronous work in 00359 versus 00650, temporal search removes the reference reversal below. Both residents favor 00359 at both speeds: its advantage spans 56--64 need-seconds at equal speeds and 40--86 after the speed change, across two calendars. Apartment order is schedule-conditioned.

The main-paper routes reconstruct 36 verified NAV transitions; plotted intersections describe spatial overlap, with simultaneous collisions outside the motion model. Earlier daily-policy examples below retain their original protocols.

\begin{figure*}[t]\centering
\begin{minipage}[t]{.48\textwidth}\vspace{0pt}\centering
\includegraphics[width=\linewidth]{figures/paired_house00685.pdf}
\captionof{figure}{\textbf{Controlled furnishing change.} The table and supported objects move together; room geometry, other furniture and start remain fixed. Cost compares complete identical needs.}
\label{fig:paired-00685}
\end{minipage}\hfill
\begin{minipage}[t]{.48\textwidth}\vspace{0pt}\centering
\includegraphics[width=.82\linewidth]{figures/frozen_temporal_comparison.pdf}
\captionof{figure}{\textbf{Frozen actors and temporal controls.} Visual summary of Table~\ref{tab:frozen-eligibility}, with 640 original needs per method under corrected timing. Actors denote distinct checkpoints; the figure summarizes their existing executions.}
\label{fig:frozen-temporal}
\end{minipage}
\end{figure*}

\textbf{Learned whole-routine comparison.} After 28 TRAIN routines in two homes, actor 6101 completes 106/108 development executions and 1,956/1,976 needs, versus its parent's 12 and 989 under identical readiness. Independent replay verifies both own-action evaluations without fallback. Of 92 complete apartment pairs, 80 are joint; four expose personal tradeoffs. Two home-work executions each leave ten needs unmet, censoring four pairs. This matched gain combines balancing and additional training.

\textbf{Whole-apartment readout.} Independent replay verifies both executions and recomputes $L_\Sigma$. Relative to 00650, home 00359 reduces residents' latency by 28.25 and 30.125 need-seconds, totaling 58.375. Movement contributes 65.575 less, witnessed forced waiting 7.2 more; other components match. Both residents benefit because shorter travel outweighs waiting. This direct joint comparison requires no solo-policy success.

Under reference execution, work at home in the same apartments changes $L_{\Sigma,A}-L_{\Sigma,B}$ from $[-363.0,-357.4]$ to $[+173.9,+177.1]$ need-seconds across two calendars when only resident~2's speed decreases from 1.20 to 0.65\,m/s. This aggregate reversal reflects opposing personal costs.


==> supplement_sections/j_final_results.tex <==
\section{Shared-layout completion, ablation, and temporal generalization}
\label{sec:final-complementarity}
\subsection{The same 50 furnishing pairs}
\paragraph{Acceptance and denominators.}
All results below come from completed independent action/event replay audits, with original-need identities and the pending-need integral checked separately. Replay verifies record consistency with the simulator; original-need checks determine routine completion. All failures and technical truncations remain in the denominators. No models were retrained for these evaluations.

\paragraph{Matched inputs.}
The static-study cohort supplies 100 furnished scenes, each executed in solo, asynchronous-pair and synchronous-pair contexts: 300 scenarios and 150 matched A/B comparisons per method. These are one- and two-resident experiments, distinct from the three-resident family series. The frozen uniform6101 actor is evaluated at update 512. Every A/B comparison matches needs, numerical profiles, release times, horizon and execution protocol. All 150 A/B pairs are explicitly bound by pair identity and context and pass the same strict input validator.

\begin{center}\begin{minipage}{\linewidth}\centering\small
\captionof{table}{Independent shared-layout outcomes. Full: all original needs completed; observed: scalar available over the declared horizon. Each row retains 300 scenarios and 5730 needs.}
\label{tab:final-pairs50}
\begin{tabular}{@{}lrrr@{}}\toprule
Executor/interface & Full & Needs met & Observed\\\midrule
Coarse navigation&27&1345&37\\
Corrected navigation&51&1770&58\\
NAV-only mask&51&1770&71\\
Request + NAV mask&51&3775&300\\
Reference planner&51&3775&300\\\bottomrule
\end{tabular}\end{minipage}\end{center}

The corrected navigation uses a 2.5-cm grid and rejects interaction through unrelated furniture. This correction changes the execution geometry while learned weights remain fixed. Repeated blocked-route actions explain the 242 technical caps after the geometry correction. Masking only NAV reduces unavailable outcomes to 229, with completed needs and full scenarios unchanged. Masking currently unreachable requests as well yields 2005 additional completed needs and no unavailable scalars under the same 12000-action limit. Each mask configuration defines an explicit deployment interface for the frozen actor. Every original request remains in the evaluation denominator. Horizon-censored scalars describe partial execution; complete matched routines support model-specific cost comparisons.

The corrected-grid reference and the request-plus-NAV executor each complete 17 scenes in all three contexts. Only pairs 009, 026, 028 and 041 have both alternatives complete in every context: 12 of 150 context-specific comparisons. All 12 have exactly zero A-minus-B household latency. The other 138 comparisons remain unsupported for complete-routine comfort ranking. The NAV-only interface also supports 12 complete comparisons; coarse navigation supports six. Thus the experiment establishes improved execution and observability; the input-equivalence check below determines how its paired outcomes can be interpreted. Residual unreachable targets and unresolved geometry retain their separate diagnostic statuses.

\paragraph{What the adapter actually distinguishes.}
A post-run inspection of all 150 saved A/B input pairs finds 36 equivalent contexts, corresponding to 12 of 50 furnishing pairs. Equality holds for runtime nodes, rooms, navigation and scenario fields after excluding identifiers and source metadata. The remaining 38 pairs have different navigation inputs. All four complete pairs belong to the equivalent subset: pair 009 rotates a balcony chair, 026 a balcony storage cabinet, and 028/041 a balcony wardrobe. Each edit reverses the front by $180^\circ$ without changing its footprint; none of these objects is referenced by an original task. The adapter preserves all source furniture and uses its footprints as obstacles, but constructs interaction fronts for task targets. These four edits preserve interaction points and routes, explaining equal delays through unchanged task-relevant runtime inputs. This motivates the task-relevant input checks used for the interventions in Appendix~H.

\subsection{Profile-by-calendar pilot on complete pairs}
A preregistered exploratory pilot conditions on the four complete pairs above. It crosses the original speed with a $0.7\times$ speed for resident~0 (1.20 to 0.84\,m/s), and original request releases with a 120-s shift for that resident. The geometry, all original requests, activities, deadlines and 7200-s horizon are unchanged; both A/B alternatives receive identical interventions. The 24 original cells are retained by audited provenance. The three new factorial cells yield 72 new scenarios, 36 new A/B comparisons, 72 reference executions and 144 independent audits. The already audited request-plus-NAV interface is fixed before observing these new outcomes; selection precedes the NAV-only ablation outcomes.

Both reference and the request-plus-NAV executor complete all 72 new scenarios, and every one of the 36 new paired latency differences is exactly zero. The original 12 paired comparisons were also tied. The source-input check explains these ties: both alternatives have equivalent task-relevant representations, and receive the same speed and release interventions. This pilot tests household-condition changes on equivalent executable layouts. Earlier profile-dependent contrasts use distinct runtime inputs and are reported separately. The four pairs form the fully complete subset of the 50-pair corpus.

\subsection{Frozen family actors at new calendar shifts}
\label{sec:calendar-extrap-final}
Eight frozen actors (paired initializations 7201--7204, synchronous-only versus diverse-calendar demonstrations) are tested at previously unevaluated 60-s and 330-s offsets. Each actor executes 288 scenarios on the same four admitted homes: three routines, six numerical profiles, two request realizations, two calendars and four homes. These are temporal generalization tests; no new geometric transfer or demographic validation is implied. The reference completes 288/288. All eight actor audits are accepted, with one distinct execution record per case.
\begin{table*}[t]\centering\small
\caption{Complete family routines at new offsets. Each offset has 144 scenarios; total denominator is 288. S: synchronous-only; D: diverse-calendar training.}
\begin{tabular}{@{}lrrrrrr@{}}\toprule
 &\multicolumn{2}{c}{60 s}&\multicolumn{2}{c}{330 s}&\multicolumn{2}{c}{Total}\\
Seed&S&D&S&D&S&D\\\midrule
7201&72&126&72&114&144&240\\
7202&72&144&84&144&156&288\\
7203&141&144&114&144&255&288\\
7204&108&108&102&108&210&216\\
\bottomrule\end{tabular}\end{table*}

Diversity increases full completion in all four paired initializations by 96, 132, 33 and 6 scenarios, respectively. The descriptive totals are 1032/1152 versus 765/1152 across repeated scenarios and paired seeds. Gain varies across seeds, with 72 outcomes still incomplete for diverse7204. Complete routines support apartment-cost comparisons; incomplete outcomes retain their policy-conditioned status.

\paragraph{Overall interpretation.}
The static, preference and dynamic studies measure complementary properties under declared conditions. Earlier complete-routine witnesses demonstrate schedule-dependent rankings and personal tradeoffs. The shared-50-pair study additionally shows why task coverage must accompany behavioral evidence: spatial rules assess furniture fronts beyond those used by a particular routine. Together, the studies motivate complementary reporting of spatial validity, preferences, need fulfillment and individual burdens, supporting interpretable choices under explicit household conditions.


==> supplement_sections/k_illustrative_layouts.tex <==
\FloatBarrier
\section{Task-covered furnishing interventions and audited trajectories}
\label{sec:illustrative-layouts}
\paragraph{Purpose and selection.}
These explanatory case studies connect a furnishing intervention to the routines that use it. They are distinct from the original 50-pair comparison. Three previously complete A scenes (009, 026, 028) supply real archived geometry; their new B variants change a task-used dining-table front, wardrobe position and sofa position, respectively. Bases are selected from cases with known completion for explanatory case studies. Before new execution, a finite protocol fixes the target, candidate order and input-only acceptance: no added floor-furniture overlap or outside-room area, all original task targets reachable, and at least 0.25\,m change in a task-node distance. The first admissible candidate is retained without consulting new policy outcomes. The first two sofa positions are rejected (overlap and outside-room placement); the third is admitted. No furniture or original need is removed.

\paragraph{Matched conditions and acceptance.}
Each new pair is evaluated in solo, asynchronous and synchronous contexts, with original speed or resident~0 slowed from 1.20 to 0.84\,m/s: 36 scenarios and 18 A/B comparisons per method. Releases are spaced every 120\,s instead of 180\,s, retaining the 180-s resident-1 offset in the asynchronous context, all task dependencies, and the 7200-s horizon. The denser request schedule defines a new evaluation condition. The frozen uniform6101 actor uses the audited request-plus-NAV interface. The checkpoint and execution interface are fixed before comparison. Both methods complete all 36 scenarios and all 660 original needs, and both independent audits pass. Every paired comparison is supported. The reference planner and learned executor yield the same paired costs on these cases.



\paragraph{What the examples add.}
The table-front reversal tests an assigned access interface on a physically symmetric table. Its 8.542--20.744 need-second differences quantify sensitivity to the assigned access side. The unequal personal differences (13.417 and 3.417 need-seconds in the synchronized normal-speed condition) remain reproducible simulator outcomes. We therefore use the directional wardrobe study below as the physically interpretable orientation example. Task coverage spans four functional rooms and hallway transit; the balcony has no assigned task. No preference reversal occurs.

The 0.40-m wardrobe and sofa translations also change runtime inputs, but their aggregate effects are small: B increases latency by at most 0.152 and 0.051 need-seconds, respectively. These small differences depend on the 2.5-cm navigation discretization and the executor's 0.2-s minimum NAV duration. Their role is to show that a visible, task-covered geometric change can have little impact under a declared routine. All examples retain the same reported static overlap/outside-room area as A. A subsequent fixed E/F rescore on these exact scenes is reported in Section~\ref{sec:efd-same-layouts}.

\paragraph{Trajectory provenance.}
Figures below use the prespecified synchronized original-speed condition for all three examples. Each plotted transition comes from an audited NAV event. Its polyline is reconstructed on the same pinned collision-free grid; the full distance matrix agrees exactly with the execution input, and every event duration agrees with $\max(0.2,d/v)$. Repeated identical routes are drawn once. Timelines retain actual action times; conflict labels require a causal event. The orange object is the sole furnishing intervention. The routes are reconstructed simulator paths.

\paragraph{Furnished views and complete routes.}
\label{sec:remaining-room3d}
The furnished views and full-apartment plans visualize the same executions. Each A/B pair shares camera, scale and lighting. Insets retain audited NAV transitions where perspective occludes paths. E, geometric Feng Shui and D are joined on these exact saved layouts (Section~\ref{sec:efd-same-layouts}); scores and route evidence retain their separate meanings. Each furnished view is followed by its complete plan and timeline.


\begin{figure*}[p]\centering
{\small
\captionof{table}{A-minus-B household pending-need latency (need-seconds). Positive values favor B. ``Slow'' changes resident~0 only. Every entry has complete original-need fulfillment.}
\label{tab:illustrative-deltas}
\begin{tabular}{lrrrrrr}\toprule
&\multicolumn{2}{c}{Solo}&\multicolumn{2}{c}{Asynchronous}&\multicolumn{2}{c}{Synchronous}\\
Intervention & Normal & Slow & Normal & Slow & Normal & Slow\\\midrule
Table front & 8.542 & 12.202 & 17.083 & 20.744 & 16.833 & 11.833\\
Wardrobe shift & -0.063 & -0.089 & -0.125 & -0.152 & -0.125 & -0.125\\
Sofa shift & -0.021 & -0.030 & -0.042 & -0.051 & -0.042 & -0.042\\
\bottomrule\end{tabular}}
\medskip
\includegraphics[width=.94\textwidth]{figures/room3d_009.pdf}
\caption{\textbf{Assigned access-side diagnostic for a symmetric table.} The depicted table geometry is identical in A and B. Only its assigned interaction side changes, marked on the plan view. The audited table-to-sofa route changes from 5.875 to 1.475\,m and household latency decreases by 16.833 need-seconds, with unequal personal reductions of 13.417 and 3.417. The measured effect concerns the assigned interaction side of the symmetric table. The separately tested directional wardrobe provides the physically interpretable facade example.}
\label{fig:room3d-009}
\end{figure*}
\begin{figure*}[tp]\centering
\includegraphics[width=\textwidth]{figures/illustrative_009.pdf}
\caption{\textbf{Assigned access-side diagnostic for a symmetric table.} Both layouts complete 22/22 needs. Reversing the table front changes access routes and reduces household latency from 2685.208 to 2668.375 need-seconds. The two residents benefit by different amounts under the declared access-side convention.}
\label{fig:illustrative-009}
\end{figure*}
\begin{figure*}[tp]\centering
\includegraphics[width=\textwidth]{figures/room3d_026.pdf}
\caption{\textbf{Wardrobe relocation: local route changes compensate.} Moving the wardrobe 0.40\,m increases bed-to-wardrobe distance from 2.30 to 2.70\,m but reduces the subsequent wardrobe-to-table route from 8.60 to 8.20\,m. The latter extends beyond the depicted room. Total walk changes from 60.625 to 60.700\,m per resident; the 0.075-m residual comes from entry-to-refrigerator navigation. Both layouts complete 22/22 needs. The 0.125 need-second household increment characterizes sensitivity at the grid and NAV-duration scale.}
\label{fig:room3d-026}
\end{figure*}
\begin{figure*}[tp]\centering
\includegraphics[width=\textwidth]{figures/illustrative_026.pdf}
\caption{\textbf{A visible relocation with a small routine effect.} The wardrobe moves 0.40\,m within its room without adding overlap. Both layouts complete 22/22 needs; latency changes from 2662.942 to 2663.067 need-seconds. The plan and timeline show the complete execution corresponding to the room view above.}
\label{fig:illustrative-026}
\end{figure*}
\begin{figure*}[tp]\centering
\includegraphics[width=\textwidth]{figures/room3d_028.pdf}
\caption{\textbf{Sofa relocation: a shorter arrival is offset by a longer departure.} The accepted 0.40-m shift reduces table-to-sofa distance by 0.275\,m and increases sofa-to-TV distance by the same amount; the dashed purple route denotes the second transition. Geometry screening had already rejected two earlier candidates for overlap or outside-room placement. The complete routine retains all 22 needs. The remaining household latency difference is 0.041667 need-seconds; a 0.025-m entry-to-refrigerator route difference is retained in the full accounting. Spatial screening prevents invalid edits; household execution determines whether a locally shorter route yields a net benefit.}
\label{fig:room3d-028}
\end{figure*}
\begin{figure*}[tp]\centering
\includegraphics[width=\textwidth]{figures/illustrative_028.pdf}
\caption{\textbf{Local circulation changes with nearly constant aggregate burden.} A permitted 0.40-m sofa shift preserves access to all task targets. Both layouts complete 22/22 needs; latency changes from 2661.958 to 2662.000 need-seconds. The full plan and timeline complement the local arrival/departure routes in the room view above.}
\label{fig:illustrative-028}
\end{figure*}

\FloatBarrier
\subsection{Directional wardrobe with tasks in every room}
\label{sec:directional-wardrobe}
A wardrobe has a functional facade and a back, making the orientation edit interpretable. We retain the archived A geometry of apartment~009 and move its bedroom wardrobe 0.65\,m south in \emph{both} alternatives, leaving access on either side. A faces the bed; B reverses the facade by $180^\circ$ at the identical position and footprint. The common relocation defines the baseline for this controlled orientation comparison. Before execution, a finite protocol fixes the candidate shifts (0.65, 0.75, 0.85, 0.95\,m); the first candidate passes independent input checks for no added overlap or outside-room placement and complete target reachability. Candidates are selected using input geometry before policy evaluation.

All original task chains are retained. Entry storage and balcony storage/rest tasks are explicitly added, so the scenario now includes functional activities in all six source rooms. The same solo/asynchronous/synchronous contexts, two numerical speed profiles, 120-s releases and 7200-s horizon produce 12 scenarios and six matched comparisons per method. The frozen actor uses the fixed request-plus-NAV interface. Both the reference planner and neural executor complete all 12 scenarios and 280/280 needs; both independent audits pass. Their paired costs agree. This controlled case study compares complementary evidence under two executors with agreeing costs.

\begin{table}[t]\centering\small
\caption{Added household latency of facade B relative to A (need-seconds). Both variants fulfill every need.}
\begin{tabular}{lrr}\toprule
Context & Original speed & Resident 0 slower\\\midrule
Solo &4.125&5.893\\
Asynchronous &8.250&10.018\\
Synchronous &8.250&8.250\\\bottomrule
\end{tabular}\end{table}

In the prespecified synchronized original-speed condition, the bed-to-wardrobe route is 2.625\,m in A and 7.675\,m in B. The subsequent wardrobe-to-table route is 0.10\,m shorter in B, yielding a net 4.95\,m additional walk per resident. Each resident incurs 4.125 additional need-seconds; household latency changes from 3452.917 to 3461.167 need-seconds, about 0.24\%. The aggregate change is modest relative to the total routine latency. Independent event checks confirm completed activities in all six rooms in both variants, including the balcony.

Footprint validity alone leaves the pair tied, directional access explains the detour, and household execution quantifies its consequences under a declared schedule. These assessments thus answer complementary questions. The simulator represents fixed front-side access and timed use; articulated door kinematics lie outside its state model. Figure~\ref{fig:wardrobe-facade} preserves the actual XY geometry and audited routes; its 3D room views use schematic furniture meshes and illustrative materials.

\begin{figure*}[tp]\centering
\includegraphics[width=\textwidth]{figures/wardrobe_room3d.pdf}
\caption{\textbf{A directional object makes the orientation effect explicit.} The existing source-geometry room renderer shows wardrobe doors in A and its back in B from the same camera. Room and furniture footprints, openings and orientation follow the archived input; heights and materials are illustrative. The plan views below show audited routes without 3D occlusion, explaining the 5.05-m bed-to-wardrobe difference. Both synchronized scenarios complete 28/28 needs. Colored edges denote the facade. Doors are represented by fixed geometry.}
\label{fig:wardrobe-facade}
\end{figure*}

\subsection{Three assessments on the identical saved layouts}
\label{sec:efd-same-layouts}

\begin{table*}[t]\centering\small
\caption{Same-layout E/F/D comparison, A $\rightarrow$ B. D is household pending-need latency in need-seconds in the prespecified synchronized original-speed condition. All needs are fulfilled. E and F use their declared score scales; D retains fulfilled-need counts.}
\label{tab:efd-same-layouts}
\begin{tabular}{lrrrr}\toprule
Intervention & E $\downarrow$ & $F_{\mathrm{geom}}\uparrow$ & D $\downarrow$ & $\Delta$D (B--A)\\\midrule
Wardrobe facade & $22\to22$ & $43.52\to43.52$ & $3452.917\to3461.167$ & $+8.250$\\
Wardrobe shift & $28\to28$ & $74.07\to74.07$ & $2662.942\to2663.067$ & $+0.125$\\
Sofa shift & $21\to21$ & $40.12\to40.12$ & $2661.958\to2662.000$ & $+0.042$\\
Assigned table side$^*$ & $20\to20$ & $43.52\to43.52$ & $2685.208\to2668.375$ & $-16.833$\\\bottomrule
\end{tabular}
\par\smallskip\footnotesize $^*$Assigned-interface diagnostic for a symmetric object. The facade study includes extra entry/balcony needs; compare D within each pair.
\end{table*}
\paragraph{Matched geometry and fixed implementations.}
We recompute static E and geometric Feng Shui on all eight saved layouts above and join the previously audited dynamic outcomes. This rescore reuses the same geometry and audited dynamic executions. The adapter retains every room polygon, furniture footprint, facing, layer and support link. Source opening endpoints are projected by at most 1\,cm to their room boundary and represented by the archived evaluator's 8-cm inward rectangles. A generic storage cabinet is explicitly mapped to its enclosed-storage front-access type. Separate checks verify source and code hashes, geometric correspondence, static facts, score arithmetic and dynamic-result identity.

E is the archived critic penalty $3n_{\mathrm{critical}}+n_{\mathrm{advisory}}$ (lower is better), accompanied by its full findings. It includes implementation-specific recommendations. $F_{\mathrm{geom}}$ uses version 3.0.0 with the original (v1) geometry predicates; the complete HANFU rubric has separate criterion definitions. Its fixed active criteria are bedroom position (F1), living-room position (F3), circulation (F5), bed/door axis (F7), and density/function (F10), with weights $(2,2,2,2,1)$ and maxima $(4,3,4,2,3)$. These version-specific F5/F10 meanings differ from CoHABIT's complete HANFU rubric. Each layout has all 15 applicable room-level ratings. We average within each criterion and normalize its mean as $(\bar f_k-1)/(m_k-1)$, then take the fixed weighted average on a 0--100 scale. The score covers the declared geometric criteria; compass and elemental attributes remain unspecified.



\paragraph{What each assessment contributes.}
E retains explicit spatial findings. For the sofa, the living-room navigability diagnostic changes from 0.812 to 0.798 while its advisory severity and total penalty remain unchanged. An aggregate E tie can coexist with changed geometric diagnostics. The assessed spatial-preference relations and all their ratings are unchanged within each pair: these interventions preserve the assessed preference categories. F records the same declared preference profile in both alternatives.

D adds routine-dependent discrimination to those static ties. In the directional wardrobe example, equal E and $F_{\mathrm{geom}}$ coexist with a verified 5.05-m access detour and 8.25 extra household need-seconds, distributed equally between residents. Adjacent route changes compensate, linking local path differences to the full-routine total. Together the views separate spatial findings, preference categories and execution consequences on the same input. They illustrate complementary evidence, without requiring every assessment to change or treating small discretization-scale residuals as established comfort differences. The F audit independently checks back support, entry view, bed/door axis, density and aggregation; circulation is evaluated by the pinned producer algorithm.

\subsection{Contrasting spatial, preference and routine evidence}
\label{sec:efd-contrasts}


Two controlled furnishing interventions in apartment~026 are selected for changed E and preference facts before observing their new dynamic outcomes. Both retain source dimensions, all objects, all needs and complete target reachability, with no added overlap or outside-room placement. Earlier candidates and their rejection reasons remain archived. These explanatory interventions share one baseline apartment. The living-room intervention shifts the sofa and a chair 0.20\,m east and the coffee table 0.20\,m east/0.50\,m south. The bedroom intervention turns the bed $180^\circ$ and shifts it 0.60\,m north.

\paragraph{Physical preference checks.}
For these pairs, $F_{\mathrm{geom}}$ uses a pinned physical-predicate revision: door-view rays stay inside the room polygon, and rear support contacts only solid source walls. The five criteria, weights and score thresholds above are unchanged. This addresses limitations of the archived v1 geometry predicates used in Table~\ref{tab:efd-same-layouts}, whose historical scores are retained with their original version. Correcting the living-room ray that crossed a concave wall changes apartment~026's baseline from 74.07 to 62.96. No new pair mixes F versions. Independent checks cover source geometry, support, wall-aware visibility, door axis, density and score arithmetic; circulation retains the pinned producer implementation. This score covers the specified geometric preference subset.

\paragraph{Matched execution and audit.}
Each intervention has six matched conditions: solo, asynchronous and synchronous routines, each with the original speed profile or resident~0 at $0.7\times$ speed. All task chains include the six apartment zones. Twelve new B cases per method are matched to twelve previously audited, hash-pinned A observations, reusing the shared baseline.  The reference planner and neural executor each fulfill 280/280 new needs in 12/12 cases, with independent audits passing; the retained A observations also fulfill every need. Explicit external-case validation checks matched needs, profiles and calendars. Both executors yield the same costs, supporting the reported furnishing contrasts under either execution method.



\paragraph{Complementarity in the living room.}
E reports reduced chair clearance (0.64 to 0.44\,m) and changed neighboring gaps; F3 separately detects lost sofa backing (rating 2 to 1). Yet the table-to-sofa route shortens from 7.10 to 4.55\,m and sofa-to-TV from 3.125 to 2.925\,m. In the synchronized original-speed routine, B reduces total latency by 7.750 need-seconds while changing individual costs by $+11.125/-18.875$. With slower resident~0, B instead adds 28.009. The solo/asynchronous deltas are $-8.354/-16.708$ at original speed and $-11.935/-20.289$ with slower R0. Static preference, geometric access and household scheduling therefore provide distinct evidence for the same choice.

\paragraph{Complementarity in the bedroom.}
E detects a 0.45-m bed--wardrobe gap and partial obstruction of wardrobe access, while the earlier door-opening finding disappears. F7 independently detects the bed facing the door axis (rating 2 to 1). Bed-to-wardrobe distance increases from 2.300 to 4.725\,m. The synchronized original-speed total increases by 19.333, but the residents' changes are $+52.167/-32.833$; with slower R0 the total changes by $-1.167$. Solo/asynchronous changes are $+3.896/+7.792$ at original speed and $+5.565/+9.461$ with slower R0. Personal accounting resolves who benefits from these simulator-specific aggregate changes. Together, the examples show household-dependent tradeoffs among the separate criteria.

\begin{figure*}[p]\centering
{\small
\captionof{table}{Matched same-input contrasts. E is a penalty, $F_{\mathrm{geom}}^{v2}$ a preference score; $\Delta$D is B--A household pending-need latency (need-seconds). The last two columns use synchronized routines.}
\label{tab:efd-contrasts}
\begin{tabular}{lrrrr}\toprule
Intervention & E $\downarrow$ & $F_{\mathrm{geom}}^{v2}\uparrow$ & $\Delta$D original & $\Delta$D slower R0\\\midrule
Living-room arrangement & $28\to34$ & $62.96\to51.85$ & $-7.750$ & $+28.009$\\
Bed rotation/shift & $28\to29$ & $62.96\to40.74$ & $+19.333$ & $-1.167$\\\bottomrule
\end{tabular}
}
\medskip
\includegraphics[width=.94\textwidth]{figures/efd_sofa_backing.pdf}
\caption{\textbf{Static preference and routine efficiency answer different questions.} Exact source footprints and orientation are rendered from a common camera; materials and heights are illustrative. Plan insets show the same audited resident's selected transitions, with full distance-matrix and event-duration checks. Both complete synchronized cases fulfill 28/28 needs and include activities in all six rooms. The living-room intervention changes three objects jointly; D measures their combined arrangement effect.}
\label{fig:efd-sofa-backing}
\end{figure*}
\begin{figure*}[tp]\centering
\includegraphics[width=\textwidth]{figures/efd_bed_axis.pdf}
\caption{\textbf{A directional bed connects placement, access and individual burdens.} Bed facing and location change together; all other furniture remains fixed. The plan view shows the audited bed-to-wardrobe transition; the preceding sink-to-bed distance includes travel outside this room. Both variants complete 28/28 needs in the illustrated condition. The accompanying data retain all six prespecified conditions, including the slower-resident profile; the figure shows the synchronized original-speed condition.}
\label{fig:efd-bed-axis}
\end{figure*}

